BandFuzz: An ML-powered Collaborative Fuzzing Framework

Collaborative fuzzing combines multiple individual fuzzers and dynamically chooses appropriate combinations for different programs. Unlike individual fuzzers that rely on specific assumptions, collaborative fuzzing relaxes assumptions on target programs, providing robust performance across various programs. However, existing collaborative fuzzing frameworks face challenges including additional computational resource requirements and inefficient resource allocation among fuzzers. To tackle these challenges, we present BANDFUZZ, an ML-powered collaborative fuzzing framework that outperforms individual fuzzers without requiring additional computational resources. The key contribution of BANDFUZZ lies in its novel resource allocation algorithm driven by our proposed multi-armed bandits model. Different from greedy methods in existing frameworks, BANDFUZZ models the long-term impact of individual fuzzers, enabling discovery of globally optimal collaborative strategies. We propose a novel fuzzer evaluation method that assesses not only code coverage but also the fuzzer's capability of solving difficult branches. Finally, we integrate a real-time seed synchronization mechanism and implementation-wise optimizations to improve fuzzing efficiency and stability. Through extensive experiments on Fuzzbench and Fuzzer Test Suite, we show that BANDFUZZ outperforms state-of-the-art collaborative fuzzing framework autofz and widely used individual fuzzers. We verify BANDFUZZ's key designs through comprehensive ablation study. Notably, we demonstrate BANDFUZZ's effectiveness in real-world bug detection by analyzing results of a worldwide fuzzing competition, where BANDFUZZ won first place.

==> ccs/1-introduction.tex <==
\section{Introduction}
\label{sec:introduction}

% BG

% The primary goal of fuzz testing is to comprehensively explore a program's state space, ensuring a thorough evaluation of its behavior across a wide range of inputs. In recent years, there has been a significant focus on research aimed at broadening the search space of programs through enhancements and optimizations of key fuzzer components. These improvements include advanced seed selection techniques~\cite{she2019neuzz,she2020mtfuzz,li2019cerebro,wang2020not,zhao2022alphuzz,wang2021reinforcement,rebert2014optimizing,liang2019deepfuzzer,herrera2021seed,gan2018collafl,zhu2023better}, more efficient power scheduling~\cite{bohme2016CoveragebasedGreyboxFuzzing,yue2020ecofuzz}, and increasingly effective input mutation strategies~\cite{rawat2017vuzzer,lemieux2018FairFuzzTargetedMutation,jauernig2023DARWINSurvivalFittest,lyu2022MOPTOptimizedMutation,aschermann2019REDQUEENFuzzingInputtoState,2023AkiHelinRadamsa,you2019profuzzer,wang2021cmfuzz,lee2023learning}, all contributing to the depth and breadth of fuzz testing capabilities.

The main purpose of fuzz testing is to thoroughly explore a program's different possible states. This ensures the program is carefully tested with a wide variety of inputs. In recent years, much research has focused on expanding the areas that fuzzers can explore in programs. This is done through improvements to key fuzzer components. These improvements include better techniques for selecting seeds~\cite{she2019neuzz,she2020mtfuzz,li2019cerebro,wang2020not,zhao2022alphuzz,wang2021reinforcement,rebert2014optimizing,liang2019deepfuzzer,herrera2021seed,gan2018collafl,zhu2023better}, more efficient power scheduling~\cite{bohme2016CoveragebasedGreyboxFuzzing,yue2020ecofuzz}, and more effective ways to mutate the inputs~\cite{rawat2017vuzzer,lemieux2018FairFuzzTargetedMutation,jauernig2023DARWINSurvivalFittest,lyu2022MOPTOptimizedMutation,aschermann2019REDQUEENFuzzingInputtoState,2023AkiHelinRadamsa,you2019profuzzer,wang2021cmfuzz,lee2023learning}. All of these help fuzz testing cover more code branches for the program under test.

% Problem statement

% However, recent research has highlighted a deceleration in the progress of fuzzing technologies~\cite{schloegel2024sok}. This trend is further supported by the latest public benchmarks~\cite{2023fuzzbenchreport} and outcomes from open competitions~\cite{liu2023sbft}, which reveal a scarcity of academic fuzzing proposals capable of surpassing the performance of industry-level tools like AFL++~\cite{fioraldi2020afl++}, introduced in 2020. Reports from the 2023 FuzzBench and the findings from competitions such as the 2023 SBFT also underscore that few fuzzers demonstrate consistently superior performance across diverse testing targets. This shortfall primarily stems from the reliance on various heuristics and assumptions in the design phase of research fuzzers, which may not consistently reflect the complexities encountered in practical fuzzing environments.

However, recent studies have shown progress in fuzzing technologies is slowing down~\cite{schloegel2024sok}. The latest public benchmarks~\cite{2023fuzzbenchreport} and results from open competitions~\cite{liu2023sbft} support this. They show a lack of new academic fuzzers that can outperform well-established industry tools like AFL++~\cite{fioraldi2020afl++} from 2020. Reports from FuzzBench\cite{2024fuzzbenchreport} and contests like 2023 SBFT Fuzzing Competition\cite{2023sbft} also highlight that few fuzzers consistently perform better than others across different test targets. This shortfall mainly comes from research fuzzers relying on various rules of thumb and assumptions during design. These may not match up well with the complexities seen in real-world fuzzing situations.


% Existing effort

% Acknowledging the limitations inherent in standalone fuzzing tools, recent research has begun to investigate the potential of collaborative fuzzing, a method that combines the strengths of multiple fuzzers into a single, cohesive approach. The logic underpinning this collaborative strategy is simple yet compelling: different fuzzers excel in exploring distinct aspects of a program's state space. By combining the unique search capabilities of various fuzzers, it becomes possible to achieve a more comprehensive and varied exploration of the program's state space, leveraging the individual advantages and insights provided by each fuzzer.

Recognizing the limitations of individual fuzzing tools, recent research has started looking into collaborative fuzzing. This approach combines the strengths of multiple fuzzers into one unified fuzzer. The reasoning behind collaborative fuzzing is straightforward but persuasive: different fuzzers are better at exploring different areas of a program's possible states. By combining the unique search abilities of various fuzzers, it becomes possible to explore more of the program's state space in a comprehensive way. 

% Previous methods and limitations

% Recent studies have shown that collaborative fuzzing solutions can outperform many individual fuzzers in effectiveness (e.g.,~\cite{osterlund2021collabfuzz,guler2020cupid,chen2019enfuzz,fu2023autofz}). However, they have not reached the same level of adoption as the more popular standalone fuzzing tools presumably due to several key issues. First, fuzzing is inherently limited by computational resources, and many collaborative approaches fail to account for these limitations, rendering them impractical for widespread use. Second, there is often a lack of efficient knowledge sharing between the fuzzers within a collaborative system, leading to duplicated efforts as different tools redundantly cover the same program areas, thereby reducing overall efficiency. Third, there is a deficiency in existing systems regarding the precise evaluation of each fuzzer's performance, which is crucial for allocating resources effectively to the most productive fuzzers. Last, some collaborative methods continue to rely on suboptimal algorithms for resource allocation, exacerbating the issue of computational resource wastage.

Recent studies have shown that collaborative fuzzers often outperform individual ones (e.g.,~\cite{osterlund2021collabfuzz,guler2020cupid,chen2019enfuzz,fu2023autofz}). However, the effectiveness of these collaborative systems greatly depends on using a lot of computing resources. For example, to do collaborative fuzzing, recently developed tools like EnFuzz~\cite{chen2019enfuzz}, CollabFuzz~\cite{osterlund2021collabfuzz}, and Cupid~\cite{guler2020cupid} all need to run multiple fuzzers at the same time. This puts a huge strain on fuzzing capabilities, especially when fuzzing is done on systems that cannot handle such heavy loads. Moreover, the high demand for computational cycles can prolong testing durations, potentially extending software development cycles and delaying product market entry.
% Wenxuan: Very promising, me likey.

To address these issues, we propose that an ideal collaborative fuzzer should have an efficient way to allocate resources among the individual fuzzers it uses. Overcoming this involves tackling three main challenges. 
%
First, establishing an effective way for the fuzzers to share knowledge is crucial. In a collaborative setting, various fuzzers may repeatedly explore the same code paths. Without a system for the fuzzers to exchange code coverage information, these overlapping efforts could waste a lot of computing resources.
%
Second, it is essential to develop a reliable method to accurately evaluate the performance of each fuzzer. Effective resource allocation depends on identifying and prioritizing the most productive fuzzers. Without an accurate evaluation system, determining which fuzzers are the most productive becomes difficult.
%
Third, avoiding greedy resource allocation strategies is indispensable. In a recent study, researchers used a greedy approach to resource allocation~\cite{fu2023autofz}. However, as we will demonstrate later in this paper, such strategies are sub-optimal and can sometimes even increase the waste of computing resources rather than reduce it.

% Our work

% WIth this mind, we introduce \sys, an innovative collaborative fuzzing framework designed to tackle the issues previously outlined through a set of strategic technical solutions, including a novel fuzzer evaluation method and the application of a multi-armed bandits (MAB) algorithm. Our approach is distinct from past efforts, although it builds upon concepts that have been explored to enhance fuzzing from various angles.

With this in mind, we introduce \sys, an innovative collaborative fuzzing framework designed to address the issues outlined earlier through a set of strategic technical solutions. This includes a novel method for evaluating fuzzers and the use of a multi-armed bandits (MAB) algorithm. Our approach is different from past efforts, although it builds upon concepts that have been explored to improve fuzzing from various angles.

% First, while traditional methods for assessing fuzzer performance have focused primarily on the ability to uncover new branch coverage, our evaluation extends beyond simple coverage metrics. \sys considers the effort required to resolve a branch, offering a more nuanced reflection of a fuzzer's effectiveness in real-world scenarios. This consideration allows for a deeper understanding of a fuzzer's operational efficiency.

First, while traditional methods for evaluating fuzzer performance have mainly focused on the ability to find new code branches, our evaluation goes beyond simple coverage metrics. \sys considers the effort required to explore a new branch, offering a more nuanced view of a fuzzer's real-world effectiveness. This consideration allows for a better understanding of a fuzzer's efficiency.


% Second, whereas previous initiatives have utilized bandit algorithms to optimize seed selection, energy distribution, and mutation scheduling, \sys adopts a broader perspective by framing the entire fuzzing task within the context of a bandit problem. Recognizing the limitations of conventional MAB approaches, we have tailored the bandit algorithm specifically for the unique challenges presented by collaborative fuzzing. This customization is detailed further in~\autoref{subsec:tech_allocate}, where we explore how \sys leverages these adaptations to address the complexities of coordinating multiple fuzzers effectively.

Second, while previous work has used bandit algorithms to optimize things like seed selection, power scheduling, and mutations, \sys takes a broader view by framing the entire fuzzing task as a bandit problem. Recognizing the limitations of conventional multi-armed bandit approaches, we have tailored the bandit algorithm specifically for the unique challenges of collaborative fuzzing. This customization is detailed further in~\autoref{subsec:tech_allocate}, where we explore how \sys leverages these adaptations to effectively coordinate multiple fuzzers.


% Characteristics

% To the best of our knowledge, this study represents the inaugural effort to design and implement a collaborative fuzzing framework that leverages a machine learning algorithm. Through meticulously planned laboratory experiments, we show that \sys not only surpasses many popular fuzzers but also significantly outperforms the latest collaborative fuzzing techniques. We took \sys to recent fuzzing competitions and were pleasantly surprised to find that it outperformed all competitors across every test. This underscores \sys's superior effectiveness, stability, and adaptability across a wide range of program types, as evidenced by its performance on FuzzBench.

To the best of our knowledge, this study is the first effort to design and implement a collaborative fuzzing framework that uses a machine learning algorithm. Through carefully designed lab experiments, we show that \sys outperforms many popular fuzzers (e.g., AFL++~\cite{fioraldi2020afl++}) and significantly outperforms the latest collaborative fuzzing techniques (e.g., autofz~\cite{fu2023autofz}). We entered \sys into recent fuzzing competitions and found that it performed better than all other competitors across every test. This highlights \sys's superior effectiveness, stability, and ability to adapt across a wide range of program types, as shown by its performance on FuzzBench.


% Summary of contributions

In summary, this paper makes the following contributions.

\begin{itemize}[leftmargin=*]

	% \item We present \sys, a collaborative fuzzing framework powered by bandit algorithms, featuring an innovative method for evaluating fuzzer effectiveness alongside a bandit-based resource allocation mechanism.

        \item We introduce \sys, a collaborative fuzzing framework. It has an innovative way to evaluate how effective each fuzzer is, along with a mechanism that uses bandit algorithm to allocate resources.

	\item We have developed \sys to incorporate 10 widely-used fuzzers, demonstrating its superiority over state-of-the-art fuzzing approaches not only in the lab setting but also in a recent fuzzing competition event.

	\item We have designed and executed a comprehensive set of experiments to assess the effectiveness of \sys, facilitating a detailed comparison with alternative fuzzing techniques.  

\end{itemize}



% % BG
% In recent years, fuzzing has emerged as a pivotal technique in software testing, drawing considerable attention from the research community. This surge in popularity is evidenced by the plethora of fuzzing strategies and tools that have been developed~\cite{zalewski2020afl, fioraldi2020afl++, fioraldi2022libafl, chen2018angora, google2020honggfuzz, bohme2016CoveragebasedGreyboxFuzzing, lemieux2018FairFuzzTargetedMutation, jauernig2023DARWINSurvivalFittest, lyu2022MOPTOptimizedMutation, aschermann2019REDQUEENFuzzingInputtoState, Lafintel2016, 2023AkiHelinRadamsa, chen22SYMSANTimeSpace}.

% The primary aim of fuzzing is to thoroughly explore a program's state space, thereby ensuring an exhaustive assessment of its behavior under diverse inputs. 
% Each fuzzer employs unique implementations of various fuzzing techniques, including seed selection, power scheduling, and mutation strategies. The majority of research in the field of fuzzing has been primarily focused on expanding the search space by refining and optimizing these techniques within fuzzers.


% % Problem statement
% Recent research has observed a slowdown in the advancements of fuzzers~\cite{schloegel2024sok}. This observation is further corroborated by recent public benchmarks~\cite{2023fuzzbenchreport} and competitions~\cite{liu2023sbft}, which highlight a lack of academic proposals for fuzzers that can outperform industry-level counterparts such as AFL++~\cite{fioraldi2020afl++}, which is initially proposed in 2020. Furthermore, it is evident from these benchmark results that few fuzzers are capable of achieving optimal performance across all targets. The reason behind this lies in the fact that researchers employ various heuristics and assumptions during their design process. Unfortunately, these may not always align with or adequately address real-world problems.

% Recognizing the constraints of our current trajectory, we opt for a different approach. Rather than developing an improved seed selection algorithm or introducing an entirely new mutation strategy, we propose a dynamic scheduling in fuzzers during the fuzzing process to enhance overall performance.
% As we believed, a more expansive and comprehensive searching space can be achieved through the integration of multiple existing fuzzers. This concept, which is referred to as ``collaborative fuzzing'', posits that by merging the distinct searching spaces of various fuzzers, we can create a synergistic effect. Such an approach allows for a broader and more diverse exploration of the program's state space, tapping into the unique strengths and perspectives of different fuzzers.

% % Previous methods and limitations
% There exists some research attempted to ensemble different fuzzers together~\cite{osterlund2021collabfuzz,guler2020cupid,chen2019enfuzz,fu2023autofz}. 
% However, these studies are not without their shortcomings. First and foremost, fuzzing is subject to computational constraints. We posit that the same limitations should be taken into account in these works as they often necessitate additional computational resources.
% Secondly, these studies employ low-frequency knowledge sharing which results in different fuzzers redundantly exploring identical program spaces. This redundancy leads to an unnecessary expenditure of resources and a decrease in fuzzing efficiency.
% Thirdly, the evaluation methodologies used for fuzzers in these studies are overly simplistic and fail to consider the potential for higher performance at later stages of fuzzer operation.
% Lastly, the design of resource allocation strategies employed by these works, either fixed or greedy, falls short when it comes to balancing exploration of different fuzzer performances with exploitation of top-performing fuzzers during task execution. This lackluster approach fails to capture real-time dynamics within the process of fuzzing, leading ultimately to sub-optimal overall performance.

% % Our work
% Despite the acknowledged limitations, our research introduces \sys, a novel collaborative fuzzing tool designed to intelligently schedule fuzzers in real-time. 
% This tool utilizes a custom multi-armed bandits (MAB) algorithm, allowing \sys to dynamically and adaptively allocate computational resources to the most effective fuzzers throughout the entire process of fuzzing for any given target programs.
% % Firstly
% \sys operates without requiring more computational resources than those integrated with existing fuzzers.
% % Secondly
% It ensures that all fuzzers receive the latest information before executing any fuzzing tasks.
% % Thirdly
% Significantly, \sys functions independently of prior knowledge; instead, it determines optimal strategies through an innovative method specifically developed for assessing fuzzer performance at runtime.
% % Fourthly
% Moreover, \sys continuously adjusts its resource allocation for fuzzing according to changes in environmental conditions. This feature enables real-time performance optimization rather than reliance on static strategies derived from offline experiments.
% We are confident that \sys will lay a solid foundation for future progress in the realm of collaborative fuzzing.


% % Characteristics
% To the best of our knowledge, this research is the first work that designs and implements a collaborative fuzzing framework powered by reinforcement learning, specifically leveraging a multi-arm bandits-based resource allocation scheme. Besides, we also argue that \sys is one of the pioneering works that introduces a new metric for evaluating fuzzer effectiveness, considering not just code coverage but also a fuzzer’s capability in solving difficult branches and breaking coverage stalls. Using \sys, we show that it is possible to integrate a real-time fuzzer evaluation mechanism effectively with the proposed metric. We demonstrate that \sys could overperform all state-of-the-art (SOTA) collaborative fuzzing frameworks, specifically \autofz, in comprehensive experiments. Last but not least, we also show that \sys excels in real-world competition by highlighting its advantages in effectiveness, stability, and adaptability across various program types on FuzzBench.

% % Summary of contributions
% In summary, this paper makes the following contributions.

% \begin{itemize}
% \item We introduce \sys, a bandits-powered collaborative fuzzing framework that integrates a new metric for fuzzer effectiveness and a multi-arm bandits-based resource allocation scheme, presenting a novel approach in the domain of software testing.
% \item We design and implement a real-time fuzzer evaluation mechanism built upon the proposed effectiveness metric, enabling dynamic and effective assessment of fuzzer performance within the collaborative framework.
% \item We conduct comprehensive experiments to demonstrate the superiority of \sys over existing SOTA collaborative fuzzing frameworks and its effectiveness, stability, and adaptability when compared with individual fuzzers on FuzzBench.
% \item We establish the potential of collaborative fuzzing, supported by multi-arm bandits and reinforcement learning, as a promising solution for constructing generic fuzzers, paving the way for future advancements in the field.
% \end{itemize}

% roadmap

% The remainder of this paper is structured as follows: \autoref{sec:bg} outlines the research background. \autoref{sec:methods} details our methodologies, including the fuzzer evaluation and resource allocation techniques. \autoref{sec:impl} describes the implementation of \sys. \autoref{sec:eval} presents \sys's evaluation results, while \autoref{sec:real-world-assessment} reports its performance in a recent competition. \autoref{sec:rw} reviews related work, and \autoref{sec:discussion} discusses current issues and future directions. The paper concludes in \autoref{sec:conclusion}.

% The rest of this paper is organized as follows. \autoref{sec:bg}
% describes the research background. \autoref{sec:methods} describes our key techniques, including our proposed fuzzer evaluation methodology and resource allocation mechanism. \autoref{sec:impl} introduces the details of implementation of a bandits-powered collaborative fuzzing framework, namely \sys, leveraging the techniques proposed in \autoref{sec:methods}. \autoref{sec:eval} summarizes the evaluation results of \sys. \autoref{sec:real-world-assessment} provides the results achieved by \sys in a recent fuzz testing competition. \autoref{sec:rw} offers a discussion of related work, followed by the discussion of some related issues and future work in \autoref{sec:discussion}. Finally, the paper is concluded in \autoref{sec:conclusion}.










%%%%%%%%%%% OLD


% This is achieved through a series of interconnected components: seed selection, power scheduling, and mutation strategies, each playing a crucial role in the fuzzing process. Each fuzzer, characterized by its unique implementation of these components, is intrinsically linked to a specific searching space within the program's state space.

% \wenxuan{Need showcase, for example bitmap} \wenxuan{must adress the "search space" is under limited resources, or same resources} This concept of a searching space represents the range and depth of program behaviors and scenarios that a particular fuzzing strategy is capable of exploring. By selecting and tailoring these strategies, researchers and developers can navigate different paths through the complex landscape of software behaviors, each path offering a unique perspective and uncovering distinct sets of potential vulnerabilities.

% In an ideal scenario, where resources are abundant, executing multiple fuzzing strategies concurrently and consolidating their findings would be straightforward. However, the reality of fuzzing often involves resource limitations, such as constrained CPU quotas and memory usage, necessitating a more strategic approach through efficient strategy scheduling. \wenxuan{Another reason for scheduling is the speed of search space expanding is not constant.} When implementing an efficient strategy scheduling method under these constraints, two primary issues come to the forefront. \textit{C1: Redundant Exploration Overlap.} The searching spaces of different strategies often intersect significantly. This leads to unnecessary duplication in the exploration of program states, as multiple strategies redundantly navigate the same aspects of the program's state space. The consequence of this overlap limits the breadth of unexplored state space that could potentially reveal undiscovered vulnerabilities, which in the end impacts the overall efficiency of the fuzzing process. \textit{C2: Dynamic Performance Variability.} Performance variability is a notable characteristic of fuzzing strategies, exhibiting variations in effectiveness across different fuzzing targets and during different periods when focusing on the same target~\cite{fu2023autofz}. Firstly, across different targets, fuzzing strategies may excel in one context but exhibit reduced effectiveness in another, requiring a nuanced approach to selecting the right strategies for collaborative fuzzing, which we refer to as "Inter-Target Variability." Secondly, when considering the same fuzzing target over different time periods, strategies may experience fluctuations in their effectiveness, with some periods yielding substantial discoveries and others seeing a decline in vulnerability identification, which we term "Intra-Target Variability." Failure to address these variabilities can lead to suboptimal resource utilization and hinder the overall success of collaborative fuzzing efforts.

% Having identified the primary issues, we outline two fundamental requirements, critical to the successful design and implementation of a collaborative fuzzing approach.

% \textbf{Real-time information sharing.} Addressing \textit{C1} necessitates the first requirement: sharing information across fuzzing strategies to reduce redundancy. In collaborative fuzzing, it is essential that all strategies share their findings and progress with each other promptly. This shared knowledge ensuring that their exploration efforts do not redundantly cover the same areas of the program's state space. By effectively disseminating this information among the strategies, each can focus on distinct, unexplored segments, thereby maximizing the efficiency and comprehensiveness of the fuzzing process and making optimal use of the available resources.

% \textbf{Real-time performance adaptation.} To effectively address \textit{C2}, a crucial requirement is the dynamic adaptation of strategy scheduling over time.  This requirement calls for a robust system capable of continuously monitoring and analyzing the effectiveness of each fuzzing strategy without solely relying on prior knowledge. The collaborative fuzzing framework must maintain adaptability and responsiveness, swiftly adjusting to performance fluctuations, and dynamically scheduling strategies based on real-time insights.



% \wenxuan{our main contribution: 1.2.3.4....}

% \wenxuan{following by the original introduction written by Jiahao.}

% In the ever-evolving domain of software security, fuzzing has established itself as a pivotal technique for uncovering hidden vulnerabilities in software applications. With the advancement of technology, the number and diversity of fuzzers are growing, each claims to improve the fuzzing performance in unique ways. However, this diversity presents a challenge: determining the most effective fuzzer for a given target program remains a complex and unresolved question. Even renowned fuzzers leading the board like AFL++~\cite{fioraldi2020afl++} have shown varying levels of effectiveness for different programs~\cite{asprone2022comparing,fioraldi2022libafl,metzman2021fuzzbench}, indicating that no single fuzzer consistently outperforms others across all programs.

% The fuzzing landscape is largely dominated by four primary types of fuzzers: AFL~\cite{zalewski2020afl}, Honggfuzz~\cite{google2020honggfuzz}, libAFL~\cite{fioraldi2022libafl}, and Angora~\cite{chen2018angora}, along with their numerous variants. Each fuzzer possesses distinct methodologies and strengths, making them uniquely suited to different testing scenarios. However, in practice, it is a daunting task to predetermine which fuzzer will be most effective for a specific target program without engaging in extensive trial-and-error testing.

% This challenge brings us to the concept of collaborative fuzzing~\cite{osterlund2021collabfuzz,guler2020cupid,chen2019enfuzz,fu2023autofz} – an approach that aims to harness the collective strengths of various fuzzers. The underlying principle is simple yet powerful: by combining different fuzzing techniques, it is possible to create a more robust and comprehensive fuzzer. However, current implementations of collaborative fuzzing adopt a rather simplistic strategy in integrating different fuzzers. To integrate different fuzzers, prior works typically choose the following approaches coming with different downsides:

% \begin{itemize}
%     \item Hand-picking combination~\cite{chen2019enfuzz}. This method involves manually selecting fuzzers to combine. However, it not only needs some expert knowledge of the fuzzers and target program but also introduces inevitable human biases, which would potentially lead to suboptimal performance.
%     \item Offline evaluation~\cite{guler2020cupid,fu2023autofz}. In this way, the fuzzer would allocate some resources to evaluate the individual fuzzer's performance offline and then prioritize the best-performing fuzzers. However, this method not only consumes valuable resources but may also struggle to adapt to the online environment when multiple fuzzers are concurrently contributing to the fuzzing process.
%     % \item Parallel running~\cite{asprone2022comparing}. In this approach, the fuzzers only support multiple cores and run in parallel. It cannot be applied to the environment where the fuzzers are running on the same core, limiting its applicability in certain environments. \jiahao{Plz check if it is right.} \wenxuan{not correct. almost every fuzzer support parallel running.}
% \end{itemize}
% In each of these approaches, the integration of fuzzers into a collaborative framework presents unique challenges that need to be addressed to optimize the effectiveness of the fuzzing process.


==> ccs/2-background-ccs.tex <==
\section{Background}
\label{sec:bg}

% Fuzzing, as an extensively explored domain, has seen a variety of research efforts ranging from the development of individual fuzzers that enhance specific fuzzing components, to collaborative fuzzing which integrates multiple fuzzers. 
% In the following, we briefly summarize these research endeavors, with a primary focus on recently emerged collaborative fuzzing frameworks and their limitations.

Fuzzing, a thoroughly studied area, covers studies from the development of individual fuzzers to systems that collaboratively use multiple fuzzers. 
Below, we concisely review recent efforts and discuss their shortcomings.

\subsection{Individual Fuzzers}
\label{subsec:bg_fuzzer}

Grey-box fuzzing research is multifaceted, focusing on improving individual fuzzer components through innovative seed selection, power scheduling, mutation strategies, and the integration of complex analysis methods.

\noindent{\bf Advanced Seed Selection. }
%
Numerous studies aim to refine seed selection strategies beyond efficiency and length, considering factors like branch behavior~\cite{she2019neuzz,she2020mtfuzz}, code complexity~\cite{li2019cerebro}, and state transition probability~\cite{bohme2016CoveragebasedGreyboxFuzzing, rawat2017vuzzer, zhao2019send, yue2020ecofuzz}. Some representative works in this area include NEUZZ~\cite{she2019neuzz}, Cerebro~\cite{li2019cerebro}, and many others~\cite{wang2020not,zhao2022alphuzz,wang2021reinforcement,rebert2014optimizing,liang2019deepfuzzer,herrera2021seed,gan2018collafl,zhu2023better}.


\noindent{\bf Power Scheduling Enhancement. }
%
Studies like AFLFast~\cite{bohme2016CoveragebasedGreyboxFuzzing} and EcoFuzz~\cite{yue2020ecofuzz} have significantly improved power scheduling.
For example, AFLFast~\cite{bohme2016CoveragebasedGreyboxFuzzing}, utilized a Markov chain model to allocate more energy towards seeds that traverse paths that are infrequently visited.%, enhancing the power scheduling in AFL++~\cite{fioraldi2020afl++}.

\noindent{\bf Novel Mutation Strategies. } 
%
This research area focuses on creating new mutation techniques and scheduling across existing mutation methods~\cite{rawat2017vuzzer,lemieux2018FairFuzzTargetedMutation,jauernig2023DARWINSurvivalFittest,lyu2022MOPTOptimizedMutation,aschermann2019REDQUEENFuzzingInputtoState,2023AkiHelinRadamsa,you2019profuzzer,wang2021cmfuzz,lee2023learning}. For example, FairFuzz~\cite{lemieux2018FairFuzzTargetedMutation} targets mutations at bytes linked to rarely executed branches, and DARWIN~\cite{jauernig2023DARWINSurvivalFittest} introduces an evolution strategy for mutator scheduling. Furthermore, MOpt~\cite{lyu2022MOPTOptimizedMutation} and AFL++~\cite{aschermann2019REDQUEENFuzzingInputtoState} propose unique strategies for mutator scheduling and mutation prioritization respectively.

\noindent{\bf Concolic Execution and Taint Analysis Integration. } 
%
Some fuzzers incorporate concolic execution~\cite{stephens2016driller,chen22SYMSANTimeSpace,poeplau2020symbolic,yun2018qsym,poeplau2021symqemu,huang2020pangolin,borzacchiello2021fuzzolic,shen2022drifuzz} or taint analysis~\cite{chen2018angora,liang2022pata,gan2020greyone,kim2020hfl} to better tackle difficult branches, enhancing efficiency in branch resolution. Some representative examples include Angora~\cite{chen2018angora}, SymCC~\cite{poeplau2020symbolic}, and SymSan~\cite{chen22SYMSANTimeSpace}, which leverage these advanced techniques to explore challenging code paths more effectively.

%
% [xxy] The following is Wenbo's version
% I don't know where these citations should go 
% @Wenxuan, Please figure it out
%
% Most research efforts in grey-box fuzzing concentrate on optimizing the individual components of state-of-the-art (SOTA) fuzzing techniques, such as American Fuzzy Lop (AFL)~\cite{zalewski2020afl}, AFL++~\cite{fioraldi2020afl++}, or libAFL~\cite{fioraldi2022libafl}. 
% At a high level, these research endeavors can be categorized into the following classes. 
% First, many studies explore more advanced seed selection metrics that consider not only seed efficiency but also other aspects~\cite{shen2022drifuzz,li2019cerebro,wang2020not,zhao2022alphuzz,wang2021reinforcement,rebert2014optimizing,liang2019deepfuzzer,she2022effective,herrera2021seed,rawat2017vuzzer,gan2018collafl,zhu2023better}, such as path uniqueness~\cite{she2022effective,zhao2022alphuzz}.
% Another line of research focuses on enhancing power scheduling~\cite{bohme2016CoveragebasedGreyboxFuzzing,yue2020ecofuzz,liang2019deepfuzzer,pham2019smart,zhang2022path,chen2022novel}.
% For example, AFLFast~\cite{bohme2016CoveragebasedGreyboxFuzzing} leverage a Markov chain model to improve the power scheduling of AFL++, prioritizing seeds with low-frequency paths.
% The third line of works designs novel mutation strategies~\cite{rawat2017vuzzer,lemieux2018FairFuzzTargetedMutation,jauernig2023DARWINSurvivalFittest,lyu2022MOPTOptimizedMutation,aschermann2019REDQUEENFuzzingInputtoState,2023AkiHelinRadamsa,you2019profuzzer,wang2021cmfuzz,lee2023learning}.
% Notably, FairFuzz~\cite{lemieux2018FairFuzzTargetedMutation} selects important bytes in a seed corresponding to rarely executed branches and prioritizes the mutations of these bytes. 
% DARWIN~\cite{jauernig2023DARWINSurvivalFittest} leverages the evolution strategy algorithm to design a novel mutator scheduling strategy.
% MOpt~\cite{lyu2022MOPTOptimizedMutation} designs another mutator scheduling strategy based on Particle Swarm Optimization (PSO). 
% RedQueen~\cite{aschermann2019REDQUEENFuzzingInputtoState} develops another method for selecting important bytes in seeds for prioritizing mutations. 
% Finally, certain fuzzers leverage concolic execution or taint analysis to enhance the efficiency of solving challenging branches~\cite{stephens2016driller,chen22SYMSANTimeSpace,poeplau2020symbolic,chen2018angora,yun2018qsym,poeplau2021symqemu,liang2022pata,huang2020pangolin,gan2020greyone,kim2020hfl,borzacchiello2021fuzzolic}.
% % Honggfuzz~\cite{google2020honggfuzz} develops and implements more comprehensive coverage metrics.

Although individual fuzzers exhibit state-of-the-art performance in specific contexts, their effectiveness can diminish under different conditions. This variability stems from the inherent design of each fuzzer, which is based on specific assumptions that may not hold for all programs. Consequently, no single fuzzer emerges as a universally optimal solution, capable of delivering consistently optimal performance across a wide array of programs.

% While individual fuzzers showcase SOTA performance under certain situations, there are cases where these fuzzers are ineffective. 
% This is because each fuzzer has its specific assumptions that will be violated against certain programs.  
% In practice, none of these fuzzers can serve as a generic fuzzing solution that consistently demonstrates SOTA performance across diverse programs. 
% 
% [xxy] shorten it. I think this analogy is not necessary. Reviewers are not in the ML community. 
% 
% This bears resemblance to the inherent characteristics of machine learning models. 
% As stated in the No Free Lunch theory~\cite{wolpert1997no}, each learning model comes with its unique assumptions, and no single model is universally suitable for arbitrary learning problems. 

\subsection{Collaborative Fuzzing}
\label{subsec:bg_rw}

Recent research is shifting focus towards collaborative fuzzing to overcome the limitations of individual fuzzers. This strategy harnesses the collective strengths of multiple fuzzers to enhance the effectiveness of fuzzing. Below, we briefly introduce existing collaborative fuzzing techniques.


\noindent{\bf EnFuzz}~\cite{chen2019enfuzz} combines six expert-selected fuzzers running simultaneously, each on a separate CPU core. A dedicated thread synchronizes seeds across all fuzzers every two minutes, ensuring a shared and updated seed set for all participants.

% \noindent{\bf EnFuzz}~\cite{chen2019enfuzz} integrates six fuzzers, which are hand-picked based on domain knowledge and experience. 
% During the fuzzing process, the selected fuzzers run in parallel, with each taking one CPU core. 
% It also uses a dedicated thread to synchronize seeds every two minutes, i.e., get a union seed set and copy it to every fuzzer.

\noindent{\bf CollabFuzz}~\cite{osterlund2021collabfuzz} retains EnFuzz's architecture and fuzzers but extends its capabilities with advanced seed synchronization policies, offering improved selection criteria for seeds and more flexible synchronization alternatives.

% \noindent{\bf CollabFuzz}~\cite{osterlund2021collabfuzz} uses the same architecture and same individual fuzzers as EnFuzz. 
% It expands EnFuzz with more seed synchronization policies, such as providing more options for what seeds to synchronize (e.g., prioritizing important seeds) and when to synchronize them (e.g., immediately upon a seed is generated). 

\noindent{\bf Cupid}~\cite{guler2020cupid} evaluates eight fuzzers offline to measure their branch coverage probabilities. Users specify the number of fuzzers, and Cupid selects the best combination to maximize branch coverage. Like EnFuzz and CollabFuzz, each fuzzer runs on a separate CPU core, with seed synchronization akin to EnFuzz's approach.

% \noindent{\bf Cupid}~\cite{guler2020cupid} 
% first conducts an offline evaluation of eight fuzzers on some pre-selected programs and records the probability for each fuzzer to cover each branch.
% The user needs to input the number of fuzzers to use. 
% Then, Cupid selects the optimal combination for the use-specified number of fuzzers, which maximizes the average branch coverage.
% Similar to EnFuzz and CollabFuzz, each selected fuzzer is assigned a single CPU core and runs in parallel. 
% Cupid uses a similar seed synchronization policy as EnFuzz.

% \noindent{\bf \autofz}~\cite{fu2023autofz} employs a dynamic two-phase method, initially distributing equal resources to fuzzers and evaluating their unique coverage ("preparation phase"). Subsequently, the "focus phase" reallocates resources based on these evaluations. This alternating pattern continues throughout the fuzzing campaign, promoting ongoing assessment and resource adjustment.

% \noindent{\bf \autofz}~\cite{fu2023autofz} is different from the approaches of EnFuzz, CollabFuzz, and Cupid. It is tailored for conducting fuzz testing under resource constraints. Specifically, it proposes a straightforward explore-exploit method for resource allocation among the fuzzers it integrates. During the exploration phase, \autofz equips all fuzzers with equal resources to evaluate their performance. In the subsequent exploitation phase, resource distribution is adjusted according to the results of the fuzzer evaluations. This cycle of exploration and exploitation alternates throughout the fuzzing process.

\noindent{\bf \autofz}~\cite{fu2023autofz} sets itself apart from the approaches utilized by EnFuzz, CollabFuzz, and Cupid through its unique design aimed at conducting fuzz testing under the constraints of limited resources. It segments a fuzzing task into time-based intervals as multiple subtasks. Each subtask undergoes two critical phases: exploration and exploitation. During each exploration phase, \autofz evenly distributes resources among all fuzzers to fairly evaluate their performance. Based on these evaluations, the subsequent exploitation phase allocates resources preferentially to fuzzers that demonstrated superior performance during the exploration phase. This allocation strategy essentially employs a greedy algorithm that uses locally optimal solutions in subtasks to approximate a globally optimal solution in the whole fuzzing task, thereby optimizing the efficiency of the overall fuzzing process.


% \noindent{\bf \autofz}~\cite{fu2023autofz} designs a two-phase approach to enable online evaluation and real-time resource allocation for individual fuzzers.
% The first phase (``preparation phase") allocates the same amount of resources to each fuzzer and evaluates them by unique coverage.
% The second phase (``focus phase") allocates CPU resources to different fuzzers according to the evaluation result in the first phase.
% The two phases are performed alternately during the whole fuzz campaign.

% \subsection{Limitations of Collaborative Fuzzing}
% \label{subsec:rw_limit}

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{sources/figs/code-example.pdf}
    \caption{An example of two individual fuzzer's code coverage on \texttt{libpcap}. 
    The dense cycle points out the branch that the corresponding fuzzer resolves. 
    }
    \label{fig:coverage_example}
\end{figure}


Despite the highlights, existing collaborative fuzzing techniques mentioned above have not achieved the same level of popularity as the widely used individual fuzzers. Below, we outline the reasons for this discrepancy.

\begin{itemize}[leftmargin=*]

    \item \noindent{\bf Requiring additional computational resources.} EnFuzz, CollabFuzz, and Cupid all require increased computational resources for fuzz testing. Subsequently, they allocate these additional resources evenly across all the individual fuzzers they encompass. This design means that any improvement in fuzzing performance is largely due to the extra resources acquired by the collaborative fuzzing approach. Consequently, these methods are not suitable for scenarios where computational resources are constrained.

    \item \noindent{\bf Infrequent cross-fuzzer knowledge sharing. } During fuzz testing, fuzzers included in \autofz and other collaborative fuzzing frameworks either do not share their path coverage or do so infrequently. This results in considerable waste of resources, as areas of the program space left unexplored by one fuzzer might have already been covered by another.

    \item \noindent{\bf Using overly simplified fuzzer evaluation to guide resource allocation. }
    \autofz assesses each integrated fuzzer based on the uniqueness of code coverage it achieves. Specifically, fuzzers that uncover more unique paths are rated more highly. However, this approach may inadvertently limit exploration to a local area of the codebase. For instance, as illustrated in~\autoref{fig:coverage_example}, AFL might achieve higher unique branch coverage than AFL++ but become confined to the input format validation phase, failing to probe into the deeper, more critical aspects of the main program logic. In contrast, AFL++ is capable of identifying critical branch with complex conditions (as seen in Line 2), enabling subsequent fuzzing processes to delve into the main program logic and potentially achieve higher branch coverage at a later stage.
    
    % \item \noindent{\bf Inefficiencies in explore-exploit resource allocation strategy. } 
    % As previously described, during the exploration phase, \autofz allocates uniform resources to all integrated fuzzers and assesses their effectiveness. Following this, in the exploitation phase, \autofz establishes a new resource allocation for each fuzzer according to the assessment, which remains unchanged until the next exploration phase. The performance of each integrated fuzzer, however, fluctuates over time during both the exploration and exploitation stages. Maintaining a static resource allocation strategy within each phase consistently results in reduced effectiveness due to the inability to adjust to the dynamic performance of the fuzzers.
    
    \item \noindent{\bf Inefficiencies in explore-exploit resource allocation strategy.}
    As previously described, \autofz explicitly separates the fuzzing task into multiple sub-tasks and formulates a fixed resource allocation strategy for each sub-task. This greedy approach fails to consider a holistic perspective.
    Furthermore, the performance of each integrated fuzzer varies over time. Persisting with a static resource allocation strategy within each phase also falls short in adapting to the dynamic performance of the fuzzers.

    % fails to adjust to the dynamic performance of the fuzzers   ----> 1. static resource allocation strategy within each phase
    %                                                2. use a greedy allocation algorithm that failed to consider sub-optimal choices which may lead to better coverage in the future
    
    % let me summarize our discussion:
    % autofz fundemental fault: saperated exploration and exploitation --> 
    %   1. waste in exploration (no cross-fuzzer knowledge sharing, overlap)
    %   2. greedy in explotation (too simple too naive, failed to consider future dynamic)
    %           ---> autofz use a greedy resource allocation algorithm which failed to adjust to the dynamic performance of the fuzzers

    % bandfuzz use bandit to merge exploration and exploitation
    
    % \item \noindent{\bf Lacking the fine-grained resource allocation capability.} Diverging from the approaches of EnFuzz, CollabFuzz, and Cupid, \autofz is tailored for conducting fuzz testing under resource constraints. Specifically, it proposes a straightforward explore-exploit method to allocate resources for the fuzzers it incorporates. At the exploration stage,  \autofz provides all fuzzers with identical resources and thus assesses their effectiveness. At the exploitation stage, \autofz allocates resources based on fuzzer evaluation results. Throughout the entire fuzzing procedure, the exploration and exploitation happen in turns. 
    
    % Once this effectiveness assessment is concluded and the next evaluation cycle has not started, the allocation of resources to the respective fuzzers is determined. However, in between evaluation cycles, the performance of each integrated fuzzer is subject to variation over time. Persisting with a fixed resource allocation strategy within  invariably leads to decreased effectiveness.

\end{itemize}




% First, existing collaborative fuzzing frameworks cannot capture~\textbf{real-time fuzzing dynamics}. 
% In other words, they are not capable of measuring and tracking the real-time changes in the effectiveness of individual fuzzers throughout the fuzzing procedure.
% Specifically, EnFuzz and CollabFuzz directly run the selected fuzzers without any evaluation mechanism for their effectiveness.
% Cupid involves an offline evaluation, where the measure of individual fuzzers remains unchanged during the entire fuzzing process.
% \autofz incorporates a preparation phase to assess fuzzers during the fuzzing process. 
% However, this mechanism is relatively inefficient and thus cannot provide real-time measurement while maintaining a decent fuzzing efficiency.
% Without monitoring the real-time changes in the individual fuzzers' effectiveness, the collaborative fuzzing framework cannot efficiently adapt its ensemble strategies to consistently maintain fuzzing effectiveness. 
% It lacks the ability to respond promptly if a fuzzer becomes less or more effective.

% Second, existing collaborative fuzzing cannot conduct effective~\textbf{real-time resource allocation} based on the fuzzing dynamics. 
% Specifically, EnFuzz, CollabFuzz, and Cupid allocate a CPU core to each fuzzer without any resource allocations during the fuzzing process. 
% As a result, these methods are unable to adapt to variations in the performance of individual fuzzers.
% \autofz indeed integrates a resource allocation mechanism to assign resources to individual fuzzers dynamically. 
% However, this mechanism has two limitations
% 1) the mechanism is not real-time given autofz's fuzzing evaluation is not real-time.
% This prevents the allocation mechanism from promptly responding to frequent and nuanced changes in individual fuzzers' performance. 
% 2) The mechanism considers only the performance of fuzzers within a specific timeframe, without accounting for any long-term effects. 
% Essentially, this method is a greedy algorithm.  
% It allocates resources based on each local period without considering potential relationships across different periods or, in other words, lacking a global assessment. 
% As demonstrated in existing works~\cite{lyu2022MOPTOptimizedMutation, bohme2017directed,lemieux2018perffuzz, kim2020maxafl} and our evaluation in \autoref{subsec:exp_result}, a decision-making process without a global perspective is likely to result in a strategy that is not globally optimal.

% Third, not every framework incorporates a \textbf{real-time mechanism for synchronizing discoveries across various fuzzers}. 
% In particular, \autofz does not conduct synchronization within preparation phase and focus phase, while other frameworks synchronize at a low frequency. 
% This lack of real-time synchronization causes significant resource wastage, as program spaces left unexplored by one fuzzer may have already been discovered by others.




























% \begin{table}[t]
% \centering
% \caption{Comparison of different collaborative fuzzing approaches. Our proposed approach, \sys, offers a comprehensive solution to the challenges faced by prior methods.}
% % Resize the table to fit the text width
% \resizebox{0.48\textwidth}{!}{%
% \begin{tabular}{lccccc}
% \toprule
%  & \textbf{EnFuzz} & \textbf{CollabFuzz} & \textbf{Cupid} & \textbf{autoFz} & \textbf{\sys}\\
% \midrule
% Supported Fuzzing Strategies & 6 & 6 & 8 & 11 & 11\\
% Auto Selection & \xmark & \xmark & \cmark & \cmark & \cmark \\
% Dynamic Scheduling & \xmark & \xmark & \xmark & \cmark & \cmark\\
% Real-time Evaluation & \xmark & \xmark & \xmark & \tmark & \cmark\\
% Single-Core & \xmark & \xmark & \xmark & \cmark & \cmark\\
% Learning-based Collaboration & \xmark & \xmark & \xmark & \xmark & \cmark\\
% \bottomrule
% \end{tabular}%
% }

% \label{tab:comparison}
% \end{table}























% Grey-box fuzzing procedure
% Grey-box fuzzing refers to the process of generating diverse testing suits to explore the state spaces of a given program to uncover vulnerabilities~\cite{zhu2022FuzzingSurveyRoadmap}.
% The goal is to maximize the program space exploration (measured by certain code coverage metrics) while minimizing the time and computational costs. 
% In this work, we focus only on user-space programs and will not consider kernel and compiler fuzzing.  
% At a high level, existing grey-box fuzzing methods leverage the genetic method~\cite{zhu2022FuzzingSurveyRoadmap} to generate and optimize fuzzing inputs for better code coverage. 
% More specifically, the fuzzing process begins by constructing \textit{an initial seed pool} with a small set of input seeds and conducting a brief dry run stage, which tests a target program using the initial seeds. 
% Subsequently, it iteratively proceeds through the following components until termination.
% The first component is~\textit{seed selection}, which ranks the current seeds in the seed pool based on a specific metric. 
% This metric typically favors seeds with a short execution time, such as the one used in American Fuzzy Lop (AFL)~\cite{zalewski2020afl}. 
% This step also eliminates redundant and low-ranking seeds from the pool that do not impact the overall coverage. 
% Following this, an \textit{energy assignment or power schedule} component determines the number of mutations to apply to each seed in the pool. 
% Subsequently, the \textit{input mutation} component generates new testing inputs by mutating each seed with the fuzzer's mutators.
% Each seed will be mutated for a certain time determined by their assigned energy. 
% High-ranking seeds will be mutated first.
% The program is then tested with the newly generated inputs, and inputs satisfying certain criteria (e.g., discovering a new path) are added to the seed pool.


==> ccs/3-tech-ccs.tex <==



\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{sources/figs/framework_1.pdf}
    \caption{The overview of \sys. In the figure, \sys manages four fuzzers. In current round $t$, the fuzzer $F_2$ is chosen. Initially, $F_2$'s seed pool contains seeds $S_1 \sim S_3$, while the global seed pool contains $S_1 \sim S_6$. After seed synchronization, $F_2$ extends its seed pool with the missing seeds and then proceeds to execute the fuzzing task, discovering new seeds $S_7$ and $S_8$. The new seeds are added to the global seed pool and evaluated to get a reward to update the probability distribution for $F_2$.}
    \label{fig:overview}
\end{figure}


\section{Key Techniques}
\label{sec:methods}

In this section, we provide a technical overview of \sys, followed by an in-depth discussion of its critical technical components.

% To address the limitations above, we design and develop \sys. 
% At the high level, we first propose a novel evaluation method for real-time measurement of fuzzing dynamics based on the coverage feedback of each individual fuzzer. 
% More importantly, we design a real-time resource allocation mechanism utilizing multi-arm bandits, which accounts for both local and global assessment.
% In the following, we start with discussing the insights behind our designs, followed by more technical details about \sys.

% \subsection{Overview of \sys}
% \label{subsec:tech_overview}

% \paragraph{Capture real-time fuzzing dynamics.}
% As discussed in ~\autoref{subsec:bg_rw}, enabling real-time measurement of individual fuzzers' effectiveness is crucial to optimize resource allocation for more effective fuzzers, thereby enhancing overall fuzzing performance.
% To achieve this, a straightforward solution is to compute the coverage of each fuzzer after every fuzzing round and use it as the effectiveness metric.
% As detailed in Section~\ref{sec:impl}, we conduct non-trivial implementation efforts to efficiently return the coverage of individual fuzzers at each fuzzing round.
% However, coverage is not a proper metric for a fuzzer's effectiveness.
% First, it is a coarse-grained metric, as different fuzzers may exhibit the same coverage.
% This makes it difficult to determine which fuzzer to prioritize when multiple fuzzers have the same coverage.
% Second, the difficulty and importance of identifying different branches varies a lot as the fuzzing proceeds.  
% As demonstrated in~\autoref{fig:coverage_example}, a unique branch (Line 2) covered by RedQueen with a complex condition carries more importance compared to other branches, as it potentially enables the exploration of main program logic.
% Fuzzers unlocking more crucial branches should be deemed more effective than those addressing simpler ones. 
% This evaluation cannot be achieved solely with coverage information.

% To address these limitations, \autofz proposes a metric that assigns a higher weight to a fuzzer if its coverage bitmap differs from other fuzzers. 
% Essentially, this metric treats unique paths discovered by each fuzzer as the difficult ones, and the fuzzer discovering more unique paths is deemed as more effective.
% This metric is computationally inefficient as it requires the comparison of individual fuzzers' bitmaps, making it difficult to conduct the real-time evaluation of fuzzing dynamics. 
% In this work, we propose a more efficient metric for measuring branch difficulty.
% As detailed in ~\autoref{subsec:tech_measure}, we employ the time required to discover each branch as the measure of its difficulty. 
% If a branch takes a longer time to be found, we consider it more challenging. 
% Unlike branch uniqueness, recording branch discovery time introduces negligible overhead, significantly enhancing efficiency.
% We integrate this metric with branch coverage and use the combined metric (denoted as~\textit{fuzzer evaluation metric}) to evaluate the effectiveness of individual fuzzers in each fuzzing round.

% \paragraph{Multi-arm bandits based resource allocation.}
% After enabling real-time evaluation of fuzzing dynamics, the next key step for effective collaborative fuzzing is to optimize resource allocation based on individual fuzzers' effectiveness. 
% Here, we discuss the single-core setup and the goal is to assign more resources to more effective fuzzers throughout the fuzzing process.
% Straightforward solutions involve either consistently selecting the best fuzzer after each evaluation or allocating a specific amount of resources to each fuzzer based on their effectiveness ranking, as employed in \autofz.
% As discussed in~\autoref{subsec:rw_limit}, such greedy solutions lack the flexibility to explore allocation strategies that may not be optimal in the current period but could lead to better performance over longer runs.
% As a result, such solutions fall short of achieving globally optimal performance throughout the entire fuzzing procedure.
% For example, in ~\autoref{fig:coverage_example}, although AFL may achieve more code coverage than RedQueen, the branch covered by RedQueen is more crucial, especially Line 2.
% %As indicated by the code in the figure, this branch contains a critical check that is closer to a new sub-space in the program, showing its higher importance than normal coverages AFL could find.
% As indicated by the code in the figure, RedQueen solves a critical check in the first line and unlocks a sub-space closer to the main program logic, showing a great potential to further explore the program in the future.
% Allocating all resources to AFL, as suggested by the greedy algorithm, would likely result in suboptimal global performance.
% Essentially, this is the problem of balancing exploitation and exploration.

% We propose to leverage the multi-arm bandit to solve this problem.
% Multi-arm bandits, or simply bandits, represent a set of algorithms that learn efficient strategies for searching and scheduling problems~\cite{wolpert1997no,russo2018tutorial,thompson1933likelihood,zhang2022matching,auer2002finite}. 
% Their objective is to strike a balance between exploiting the current optimal choices (exploitation) and exploring for potentially better choices (exploration). 
% Bandits naturally align with our problem of balancing the exploitation and exploration in resource allocation. 
% Furthermore, in contrast to other learning problems, bandits do not require pre-collection of a dataset or training a substantial number of parameters. 
% Their real-time and efficient nature further sets them as a natural fit for our problem.
% As we will detail in~\autoref{subsec:tech_allocate}, we build a customized bandit model for our problem, which treats individual fuzzers as an arm and our proposed fuzzer evaluation metric as the reward. 
% We leverage the Thompson sampling algorithm to determine the weights for individual fuzzers in each fuzzing round and dynamically allocate resources in real time based on these weights.

% \paragraph{Overall procedure of \sys.}
% As demonstrated in~\autoref{fig:overview}, in each round, given a weight distribution of individual fuzzers, \sys first sample a fuzzer $F_2$ based on this distribution (i.e., $F_2$ is selected in round $t$) (\ding{192}).
% It then conducts a seed synchronization (\ding{193}), updating the seed pool of $F_2$ by incorporating the global seed pool (i.e., the union set of seeds from all fuzzers).
% \sys then runs $F_2$ for a certain cycle, in which each cycle performs the seed selection, energy assignment, and mutations of $F_2$ (\ding{194}).
% After fuzzing with $F_2$, \sys updates the global seed pool with the newly discovered seeds (\ding{195}) and recomputes the reward of individual fuzzers using our proposed fuzzer evaluation metric (\ding{196}). 
% Finally, \sys updates the weight distribution based on the reward using the Thompson sampling algorithm (\ding{197}).
% \sys continuously performs this iterative process until a predefined stopping criterion is reached.

% 
% 
% 

\subsection{Technical Overview}
\label{subsec:tech_overview}

To address the challenges faced by existing collaborative fuzzing techniques, we introduce \sys, a collaborative fuzzing framework powered by bandit algorithms. The high-level workflow of \sys is depicted in \autoref{fig:overview}. 

In this bandits-powered framework, each fuzzer operates as an "arm" within the bandit algorithm context. The algorithm assigns a probability distribution to each arm, and selects a fuzzer for testing based on the highest value drawn from this distribution (\ding{192}).

\sys maintains a global seed pool that aggregates the seeds discovered by each individual fuzzer. Before initiating fuzz testing, \sys compares the selected fuzzer's seed pool with the global pool. If the global pool contains seeds absent in the fuzzer's pool, \sys synchronizes these seeds, thereby enhancing the fuzzer's pool (\ding{193}).

The fuzzer then proceeds to test using the seeds from its updated pool for a brief period (\ding{194}). Should the fuzzer uncover new coverage areas, it incorporates the corresponding seeds into both its own and the global seed pools (\ding{195}).

Subsequently, \sys employs a novel method to evaluate the fuzzer's performance, assigning rewards based on the newly discovered seeds (\ding{196}). Armed with this reward, \sys adjusts the probability distribution for the fuzzer's corresponding arm (\ding{197}) and concludes a fuzzing round (i.e., \ding{192}$\sim$\ding{197}).

For a given fuzzing task, the fuzzing round iterates, updating the selection of fuzzers, until a specific predetermined condition is satisfied, such as the exhaustion of a predefined time budget.

The design of \sys effectively addresses the issues highlighted in \autoref{subsec:bg_rw}.
%
First, \sys operates efficiently within limited computational resources, distributing these resources among the integrated fuzzers without needing extra resources like some other frameworks.
%
Second, by utilizing a global seed pool for coverage sharing, \sys greatly reduces the chance of different fuzzers redundantly exploring the same areas of code.
%
Third, our fuzzer evaluation methodology, explained in \autoref{subsec:tech_measure}, considers both branch coverage and the effort required to solve the constraint of the branch, providing a more accurate reflection of a fuzzer's effectiveness in exploring code spaces.
%
Fourth, \sys employs bandit algorithms to automatically balance between exploration and exploitation, avoiding the resource-heavy exploration phases common in other frameworks. Moreover, it adeptly tracks the performance dynamics of each arm, enabling real-time adjustments in resource allocation, and thereby enhancing the overall resource allocation efficiency.
% 
In the following session, we delve into the architecture of two pivotal elements upon which \sys is built: a novel fuzzer evaluation methodology and our resource allocation mechanism, powered by bandit algorithms.
\vspace{-2mm}
%
\begin{algorithm}[t]
    \caption{Assign reward to a selected fuzzer}
    \label{alg:evaluate}
    \SetAlgoLined
    \KwIn{The current fuzzing round $t$, the selected fuzzer $F_t$, the set of new seeds generated by this fuzzer $\mathcal{S}_t$, the maximum and minimum reward $r_{\text{max}}$ and $r_\text{min}$, and the set $\mathcal{I}$, recording the round at which each basic block is \textit{firstly} discovered.}
    $r_t \leftarrow 0$\;
    \For{seed $S$ in $\mathcal{S}_t$}{
        \For{new branch $b$ covered by $S$}{
        Suppose the branch $b$ goes from the basic block $BB_p$ to $BB_e$\;
        Find the round that $BB_p$ is firstly discovered in $\mathcal{I}$, noted as $t_p$;
        Compute the coverage interval $c$ $\leftarrow$ $t - t_p $\;
        Update the reward $r_t \leftarrow r_t + c$\;
        \If{$BB_e$ is newly discovered}{
        Add the pair $BB_e$ and $t$ to $\mathcal{I}$;
        }
            }
        }
    $r_{\text{max}} \leftarrow max(r_{\text{max}}, r_t)$\;
    $r_{\text{min}} \leftarrow min(r_{\text{min}}, r_t)$\;
    $r_t \leftarrow (r - r_{\text{min}}) / (r_{\text{max}} - r_{\text{min}})$\;
    \KwOut{normalized reward $r_t$}
\end{algorithm}
%

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{sources/figs/branch.pdf}
    \caption{Motivating example for demonstrating reward computing.}
    \label{fig:evaluate}
    \vspace{-4mm}
\end{figure}


\subsection{Fuzzer Evaluation Methodology}
\label{subsec:tech_measure}

As described above, we introduce a novel fuzzer evaluation approach designed to gauge the performance of fuzzers and subsequently allocate rewards accordingly. In our framework, a high reward signifies a fuzzer's effectiveness. Below, we detail our evaluation methodology and the associated reward scheme.

To evaluate a fuzzer's performance, we consider not only its capability to uncover new branches but also the effort required to achieve such discoveries. This consideration stems from an observation that, during the initial stages of fuzzing, individual fuzzers generate a large number of seeds, contributing to an increase in coverage. However, as time progresses, identifying new branches becomes increasingly difficult, often leading to a stagnation in coverage growth. At this point, while most fuzzers face challenges in discovering new branches despite numerous mutation attempts, a select few manage to overcome complex constraints, generating seeds that unlock critical branches (as shown in \autoref{fig:coverage_example}). This breakthrough leads to a rapid emergence of new seeds, facilitated by the resolution of complex constraints and the subsequent ease of discovering additional branches.

Following this observation, we design our fuzzer assessment mechanism and reward scheme as follows. After running the selected fuzzer $F_t$ at the fuzzing round $t$, we obtain a set of new seeds, represented as $\mathcal{S}_t$.
The reward of the selected fuzzer, denoted as $r_t$, is equal to the accumulated rewards of all seeds $S \in \mathcal{S}_t$.
Each seed's reward is subsequently calculated from the accumulated rewards of all unique and newly covered branches ($b$) that are associated with it.
As indicated from Line 4 to Line 6 in~\autoref{alg:evaluate}, each branch's reward corresponds to its coverage interval ($c$). The latter quantifies how many rounds were required to discover this new branch.
Mathematically speaking, coverage interval $c$ equals the difference between the current round number ($t$) and when its preceding block (denoted as $BB_p$) was \textit{firstly} discovered.
We calculate $r_t$ by summing up values of $c$ over all newly covered branches across all seeds in $\mathcal{S}_t$.
Finally, we normalize $r_t$, using min-max scaling, to determine the final reward for fuzzer $F_t$ (Line 12-14). 
This approach allows us not only to capture overall coverage through the accumulation of newly discovered branches but also to account for the effort required via the computation of individual branches' coverage interval $c$.

% For a clearer comprehension of our reward assignment methodology, we direct readers to \autoref{appendix:reward_example}. This section includes a detailed example that demonstrates the calculation of $r_t$ for a straightforward program, facilitating a deeper understanding of the process.


\noindent{\bf Example of reward computing.}
% To enhance the comprehension of how \autoref{alg:evaluate} functions, we refer to a specific example depicted in \autoref{fig:evaluate}.
As demonstrated in~\autoref{fig:evaluate}, the program features a target program with eight distinct branches.
Initially, seed $X$ identifies branches $b_1$, $b_4$, and $b_7$ during iteration $I_X$, leading to the inclusion of $\{BB_1=I_X, BB_2=I_X, BB_5=I_X, BB_6=I_X\}$ in set $I$.
Following a series of iterations without new discoveries, seed $Y$ emerges in round $t=I_Y$, detecting branches $b_2$, $b_5$, and $b_7$, with $b_2$ and $b_5$ being newly identified.
For branch $b_2$, $BB_1$ is recognized as the preceding block ($BB_p$) and $BB_3$ as the subsequent block ($BB_e$), resulting in a coverage interval calculation of $c = t - t_p = I_Y - I_X$. Consequently, $\{BB_3=I_Y\}$ is appended to set $I$.
Regarding $b_5$, $BB_3$ is the preceding block and $BB_5$ is the subsequent block, leading to a coverage interval of $c = I_Y - I_Y = 0$.
Since $BB_5$ was previously discovered, set $I$ remains unchanged.
The fuzzer that generates seed $Y$ is then awarded a reward $r_t = (I_Y - I_X) + (0) = I_Y - I_X$.
After additional rounds without findings, seed $Z$ is identified at round $t=I_Z$, uncovering new branches $b_3$, $b_6$, and $b_8$.
The coverage interval for $b_3$ is calculated as $c = I_Z - I_X$, with $\{BB_4=I_Z\}$ added to set $I$.
The interval for $b_6$ is $c = I_Z - I_Z = 0$, and for $b_8$, it is $c = I_Z - I_X$, leading to the inclusion of $\{BB_7 = I_Z\}$ in set $I$.
Ultimately, the fuzzer that generates seed $Z$ is awarded a reward $r_t = (I_Z - I_Y) + (0) + (I_Z - I_X) = 2I_Z - I_Y - I_X$.






% In addition, it only requires maintaining an extra set $\mathcal{I}$, which introduces negligible computational and storage overhead. 

% GPT version
% Building on the observation mentioned earlier, we have crafted our fuzzer evaluation mechanism and reward scheme as detailed below. After executing the selected fuzzer $F_t$ in fuzzing round $t$, we obtain a set of new seeds generated by $F_t$, represented as $\mathcal{S}_t$.
% The reward for $F_t$, denoted $r_t$, is determined by summing up the rewards for all seeds $S \in \mathcal{S}t$.
% The reward for each seed $S$ is derived from the aggregate reward of all unique and newly covered branches $b$ by $S$.
% As outlined in Lines 4 to 6 of \autoref{alg:evaluate}, the reward for each branch $b$ is based on the coverage interval $c$, reflecting the number of rounds needed to uncover the new branch $b$.
% Mathematically, $c$ is the difference between the current round $t$ and the round in which the predecessor node $BB_p$ was first discovered.
% After aggregating $r_t$ across all branches for all seeds in $\mathcal{S}t$, \autoref{appendix:reward_example} illustrates the computation of $r_t$ for a simple program.
% Subsequently, we adjust the global maximum and minimum rewards ($r{\text{max}}$ and $r{\text{min}}$) and normalize $r_t$ using min-max scaling to determine the final reward for $F_t$ (Lines 9-11).
% This reward methodology not only encompasses coverage by aggregating all newly discovered branches but also reflects the effort involved by calculating the coverage interval $c$ for each branch.
% Moreover, it entails maintaining an additional set $\mathcal{I}$, which imposes minimal computational and storage overhead.

%
\begin{algorithm}[t]
    \caption{\sys resource allocation}
    \label{alg:fuzzer_selection}
    \SetAlgoLined
    \KwIn{A set of individual fuzzer $\mathcal{F}$, global seed pool $\mathcal{S}_{g}$, reset interval $I_R$, time budget for each round $T_I$, stopping condition}
     $timer \leftarrow 0$, Number of round $t \leftarrow 0$\;
     \For{fuzzer $F$ in $\mathcal{F}$}{
     $F.total\_duration \leftarrow 0$, $F.num\_selection \leftarrow 0$ \;
     $F.cycles \leftarrow 1$\;
     $\alpha_F$ $\leftarrow$ 1, $\beta_F$ $\leftarrow$ 1\;
     }
     \While{stopping condition is not met}{
        Current fuzzer $ F_t \leftarrow$ TS($\mathcal{F}$) (\ding{192})\;
        Synchronize seeds from $\mathcal{S}_g$ to the seed pool of $F_t$ (\ding{193})\;
        $start \leftarrow$ current time\;
        \For{$j$=0, $j$<$F_t.cycles$, $j$++}{
            $F_t$.run\_one\_cycle() (\ding{194})\;
        }
        Update $\mathcal{S}_{g}$ with $\mathcal{S}_t $, new seeds generated by $F_t$  (\ding{195})\; 
        $d_t \leftarrow$ current time $- start$, $r_t \leftarrow$ evaluate $F_t$ with~\autoref{alg:evaluate}  (\ding{196})\;
        \tcp{Update probability distribution (\ding{197})} 
        $\alpha_{Ft}  \leftarrow \alpha_{Ft} + \hat{r}_t$, $\beta_{Ft}  \leftarrow \beta_{Ft} + (1 - \hat{r}_t)$\;
        \tcp{Auto-cycle}
        $F_t.total\_duration \leftarrow F_t.total\_duration+d_t$\;
        $F_t.num\_selection \leftarrow F_t.num\_selection + 1$ \;
        $F_t.avg\_cycle\_time$ $\leftarrow$ $ \text{floor} (\frac{F_t.total\_duration}{F_t.num\_selection}$)\;
        $F_t.cycles \leftarrow \frac{T_I}{F_t.avg\_cycle\_time}$\;
        \tcp{Reset mechanism}
        $timer \leftarrow timer + d_t$, $t \leftarrow t+1$ \;
        \If{$timer \geq I_R$}{
            $timer \leftarrow 0$,               $\alpha_F$ $\leftarrow$ 1, $\beta_F$ $\leftarrow$ 1 for every fuzzer\;
            }
        }
\end{algorithm}
%

\subsection{Resource Allocation Mechanism}
\label{subsec:tech_allocate}

As outlined in \autoref{subsec:tech_overview}, our approach formalizes resource allocation using a bandits model. Within this model, the ensemble of fuzzers integrated into \sys is represented by $\mathcal{F}$, with each individual fuzzer $F\in \mathcal{F}$ conceptualized as an arm, each equipped with a probability distribution. Following the completion of each fuzzing round, \sys recalibrates the probability distribution for each fuzzer based on the rewards garnered from the previously described fuzzer performance evaluation method. For updating these probability distributions, we have chosen the Thompson Sampling algorithm (TS)~\cite{thompson1933likelihood}, applying specific customizations to better suit our needs. In the following discussion, we delve into the application of the Thompson Sampling algorithm within the context of collaborative fuzzing, detailing our customized adaptations. This is followed by an examination designed to affirm that our model remains consistent with the core principles underlying the bandits algorithm.

% As discussed in \autoref{subsec:tech_overview}, we design our resource allocation mechanism based on the multi-arm bandits model.
% Multi-arm bandits can balance exploitation and exploration towards achieving a globally optimal strategy.
% In addition, it is computationally efficient, making it well suitable for our problem. 
% At a high level, in each fuzzing round, our resource allocation mechanism first uses our customized bandits model to select a fuzzer.
% Then it leverages our proposed auto-cycle method to determine the duration for running the selected fuzzer in this round.
% In the following, we first introduce our customized bandits model and the auto-cycle method, followed by a full version of the resource allocation algorithm.


% As outlined in \autoref{subsec:tech_overview}, our resource allocation mechanism is designed based on the multi-arm bandits model. This model effectively balances exploitation and exploration, thereby facilitating the achievement of a globally optimal strategy. Moreover, its computational efficiency makes it particularly suitable for our problem.
% At a high level, during each fuzzing round, our resource allocation mechanism initially employs our customized bandits model to select an appropriate fuzzer. Subsequently, it utilizes our proposed auto-cycle method to determine the duration for running the selected fuzzer within this round.
% In what follows, we first introduce both our customized bandits model and the auto-cycle method. A comprehensive version of the resource allocation algorithm will then be presented.


% Given a set of selected fuzzers $\mathcal{F}$, we construct a customized bandit model, In this model, each arm represents an individual fuzzer $F\in \mathcal{F}$.
% Initially, each arm is equipped with a weight distribution.
% During each round of fuzzing, an arm (i.e., a fuzzer) is selected based on the current distribution.
% Subsequently, the chosen fuzzer operates for a specified duration.
% The effectiveness of this operation is then evaluated using the metric outlined in~\autoref{subsec:tech_measure}.
% We use this evaluation as the reward for the bandits model.
% Our goal is to keep updating the weight distributions in a way that maximizes the long-term accumulated reward obtained through repeated pulls of the arms.
% By maximizing the long-term reward, the bandits can select the fuzzer benefiting the overall fuzzing campaign.
% In contrast, the greedy method selects the fuzzers with the highest reward at each time but may not result in an optimal long-term reward.

% As is mentioned in~\autoref{subsec:tech_overview}, \sys formalizes resource allocation as a bandits model. In this model, the fuzzers enclosed in \sys are denoted as $\mathcal{F}$. Each arm symbolizes an individual fuzzer $F\in \mathcal{F}$ and is initially equipped with a weight distribution. 
% The fuzzing process operates in rounds. At each round, we select an arm (i.e., a fuzzer) based on the current weight distribution. The chosen fuzzer then operates for a predetermined duration.
% Following the operation of the fuzzer, we evaluate its effectiveness using the metric outlined in~\autoref{subsec:tech_measure}. This evaluation serves as the reward for our bandit model.
% Our primary objective is to continually update these weight distributions to maximize long-term accumulated rewards obtained through repeated pulls of arms and evaluation. By focusing on maximizing long-term rewards, we can ensure that our bandits consistently select the most beneficial fuzzer for overall fuzzing campaigns.


% We use the Thompson sampling algorithm (TS)~\cite{thompson1933likelihood} to update the weight distributions.
% The reason for selecting TS is it has been theoretically and empirically demonstrated to be better than other methods across various problems~\cite{russo2018tutorial,chapelle2011empirical}. 
% Suppose the fuzzer set $\mathcal{F}$ contains $K$ fuzzers.
% For each fuzzer (or arm) $F_k$, TS defines the conditional distribution for the reward as a Bernoulli distribution parameterized by $\theta_{Fk}$.
% Recall that in \autoref{subsec:tech_measure} we use $r_t$ to denote the reward of $F_t$. So $r_t | F_k \sim \text{Bern}(\theta_{Fk})$.
% TS then defines the distribution of $\theta_{Fk}$ as a Beta distribution, parameterized by $\alpha_{Fk}$ and $\beta_{Fk}$, i.e., $\theta_{Fk} \sim \text{Beta}(\alpha_{Fk}, \beta_{Fk})$.
% This is the weight distribution for $F_k$.
% In each fuzzing round $t$, TS first samples $\theta_{Fk}$ from the current weight distribution for each fuzzer.
% Then, it selects the fuzzer with the largest $\theta_{Fk}$, i.e., $F_t = \text{argmax}_{Fk} \theta_{Fk}$.
% After running the selected fuzzer and collecting the reward $\hat{r}_t$, TS then updates the parameters of the weight distribution of the selected fuzzer as follows:
% %
% \begin{equation}
% \alpha_{Ft} \leftarrow \alpha_{Ft} + \hat{r}_t, \ \ \beta_{Fk} \leftarrow \beta_{Fk} + 1 - \hat{r}_t \, .
% \label{eq:beta}
% \end{equation}
%

\noindent{\bf TS algorithm.}
% 
The TS algorithm was selected for our application due to its proven theoretical and empirical advantages over alternative methods across a diverse range of scenarios, as documented in the literature~\cite{russo2018tutorial,chapelle2011empirical}.
%
Assuming our fuzzer set, $\mathcal{F}$, consists of $K$ fuzzers, TS models the reward conditional distribution for each fuzzer (or arm) $F_k$ as a Bernoulli distribution, parameterized by $\theta_{Fk}$.
% 
As mentioned in \autoref{subsec:tech_measure}, the reward for fuzzer $F_t$ is denoted by $r_t$; hence, we have $r_t | F_k \sim \text{Bern}(\theta_{Fk})$.
%
Furthermore, TS defines the distribution of $\theta_{Fk}$ as a Beta distribution, which is parameterized by $\alpha_{Fk}$ and $\beta_{Fk}$; thus, we have  $\theta_{Fk} \sim \text{Beta}(\alpha_{Fk}, \beta_{Fk})$. This Beta distribution represents the probability distribution for $F_k$.
%


During each fuzzing iteration, indexed by $t$, TS algorithm begins by drawing a sample $\theta_{Fk}$ from the current probability distribution of each fuzzer. It then identifies and selects the fuzzer with the highest sample value, denoted as $ F_t = \text{argmax}_{ F_k }   {\theta}_{ F_k } $. Upon the execution of the chosen fuzzer and the acquisition of its resultant reward ${\hat { r }}_ t$, TS proceeds to update the parameters of this fuzzer's probability distribution. This update is facilitated through the application of the following equation:
%
\begin{equation}
\begin{aligned}
{\alpha}_{ Ft }   & {\leftarrow}{\alpha}_{ Ft } + {\hat { r }}_ t \, , 
\\ 
{\beta}_{ F_k }  & {\leftarrow}{\beta}_{ F_k } + 1 - {\hat { r }}_ t \, . 
\end{aligned}
\label{eq:beta}
\end{equation}
%

%
\begin{algorithm}[t]
    \caption{Customized TS bandit algorithm}
    \label{alg:customized-ts}
    \SetAlgoLined
    \KwIn{}
    $r_t \leftarrow 0$\;
    \For{\(t = 1, 2, \ldots\)}{
      \tcp{sample model}
      \For{\(k = 1\) \KwTo \(K\)}{
        Sample \(\hat{\theta}_k \sim \text{Beta}(\alpha_k, \beta_k)\)
      }
      \tcp{select and apply action}
      \(x_t \leftarrow \arg\max_k \hat{\theta}_k\) \\
      Apply \(x_t\) and observe \(r_t\) \\
      Sample \(\hat{r_t} \sim \text{Bern}(r_t)\) \\
      \tcp{update distribution}
      \((\alpha_{x_t}, \beta_{x_t}) \leftarrow (\alpha_{x_t} + \hat{r_t}, \beta_{x_t} + 1 - \hat{r_t})\)
    }
\end{algorithm}
%

\noindent{\bf Customizing TS algorithm.}
Using the TS algorithm mentioned above for our problem, we confront two critical challenges. The first challenge arises from the fact that TS assumes $\hat{r}_t\in\{0, 1\}$ is discrete. However, in our design, the reward $r_t$ falls within a continuous range of $[0, 1]$. To overcome this discrepancy, we employ a method proposed by Agrawal et al.~\cite{agrawal2012analysis}, which facilitates the discretization of our continuous reward $r_t$ into a binary equivalent $\hat{r}_t$. This discretized reward is then used to update the parameters following \autoref{eq:beta}, aligning our implementation with the TS framework.

Beyond the challenge of discretizing rewards, the Thompson Sampling (TS) algorithm operates under the assumption that reward distributions are static over time. However, our context deviates from this assumption as the discovery of new program branches leads to dynamic changes in reward distributions. To adeptly manage these fluctuations, we implement a strategy of periodically resetting the probability distribution parameters for each fuzzer. This method enhances our model's adaptability, enabling it to accurately reflect the evolving nature of reward distributions, as the parameters themselves are derived from the probability distribution. 
A full algorithm is shown in~\autoref{alg:customized-ts}.
For a comprehensive exploration of our tailored TS approach and an in-depth discussion on the progression of probability distribution throughout a fuzzing campaign, please see \autoref{appendix:thompson_example}.


% In addition to the discrete problem, TS also presumes that reward distributions remain stationary over time.
% However, in our scenario as more program branches are discovered over time, these reward distributions will change accordingly. In order to account for such variations effectively, we periodically reset each fuzzer's weight distribution parameters. This approach provides flexibility in capturing changes in the evolving reward distributions since its parameter is sampled from the weight distribution itself. For further details on our customized TS method and an analysis of how weight distribution evolves throughout a fuzzing campaign refer to~\autoref{appendix:thompson_example}.


\noindent{\bf Preserving the core principles of bandits with the auto-cycle mechanism.}
The bandits model operates on a fundamental principle: the reward assigned to each option, or ``arm'', must be based on similar conditions. In the context of our bandits model for collaborative fuzzing, this principle translates to ensuring that when \sys evaluates different fuzzers during a specific fuzzing round, each fuzzer is allocated a comparable amount of CPU resource. A direct approach to achieving this is by allocating a fixed duration in each fuzzing round for the selected fuzzer. However, this method poses a significant challenge: a fuzzer could be in the midst of processing a seed when the allocated time expires, potentially leaving the energy for that seed unexhausted. Interrupting the fuzzer at this juncture could compromise the integrity of the fuzzing process.

To address this issue, we propose an auto-cycle mechanism. To lay the groundwork for this solution, we first introduce the concept of a fuzzing cycle, defined as the estimated time required to execute a seed and utilize the designated energy for that seed. Given that different fuzzers operate at varying speeds and explore different paths, the duration of a fuzzing cycle can vary across fuzzers. The auto-cycle mechanism aims to ensure that \sys can provide each specific fuzzer with enough CPU resources to complete at least one full fuzzing cycle. To do this, it starts by estimating the average duration of a fuzzing cycle for each fuzzer. Based on this estimate, our mechanism calculates a fixed time budget $T_I$, which determines the number of cycles a fuzzer can perform in a single fuzzing round. This calculation is represented mathematically as $\frac{T_I}{F.avg\_cycle\_time}$, where $F.avg\_cycle\_time$ denotes the estimated time a fuzzer $F$ needs to complete a fuzzing cycle.


% After selecting a fuzzer in each round, we also need to determine its runtime, i.e., the allocated resources. 
% The principle is to maintain fairness by assigning a similar resource in each round. 
% This aligns with the bandits model assumption that rewards in each round are obtained under similar resources.
% A straightforward approach is to allocate a fixed run time for each round. 
% Unfortunately, this will break the fuzzing procedure of individual fuzzers. 
% Instead, we specify the number of fuzzing cycles to run (One cycle means the full procedure from seed selection to generating new seeds), which better maintains the fuzzing procedure. 
% Assigning the same number of cycles is also not an ideal approach, as some fuzzers operate faster than others, leading to unfairness.
% To address this, we propose the auto-cycle mechanism, which dynamically adjusts the number of fuzzing cycles for each fuzzer based on its previous run time.
% Specifically, for each fuzzer, we first calculate its average runtime in each cycle ($F.avg\_cycle\_time$).

% After choosing a fuzzer in each round, it is also necessary to determine the time resources allocated to it. The guiding principle here is fairness; we aim to assign similar resources in each round. This approach aligns with the assumption of the bandits model that rewards are obtained under similar resource conditions in every round.
% A simple method would be to allocate a fixed time for each round. However, this strategy could disrupt the individual fuzzing procedures of different fuzzers. Instead, we define the number of fuzzing cycles that should be executed; here, one cycle refers to the entire fuzzing process that starts with choosing a seed and ends before the next seed is going to be selected.
% This method more effectively maintains the integrity of individual fuzzing procedures.
% Assigning the same number of cycles is also not an ideal approach, as some fuzzers operate faster than others, leading to unfairness. To address this issue, we introduce an auto-cycle mechanism that dynamically adjusts the number of fuzzing cycles for each fuzzer based on its previous execution time.
% Specifically for each fuzzer, we first calculate its average cycle time ($F.avg\_cycle\_time$). We then establish a fixed time budget $T_I$, which determines how long a fuzzer can run in any given round. The number of cycles is computed as $T_I / F.avg\_cycle\_time$.


\noindent{\bf Resource Allocation via \sys.}
Following the introduction of the customized bandits model and auto-cycle mechanism, we now provide a formal description of \sys's resource allocation as depicted in \autoref{alg:fuzzer_selection}.
Given the necessary inputs, we commence by initializing the required variables (Lines 1-6).
In each fuzzing round, our first step is to select fuzzer $F_t$ utilizing our tailored bandits model (Line 8), followed by synchronizing its seeds with those in the global seed pool (Line 9).
Subsequently, we execute $F_t$, gather its reward, and update both its probability distribution and the global seed pool (Lines 10-16).
We also employ the auto-cycle mechanism to revise how many cycles a fuzzer should run when it is selected next time (Lines 17-20).
Last, after updating the model for certain rounds, we reset parameters within our bandits model to ensure optimal performance moving forward (Lines 21-24).




































%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                             OLD STUFF                                           %
%                                                                                 %

% \wenxuan{fuzzing is not pure stochastic. we need to reset.}
% To begin, the TS algorithm exhibits a slow response to evolving trends, potentially favoring early-selected fuzzers that achieve significant coverage improvements. This bias might overshadow more effective fuzzers.

% %Firstly, in the initial stage of the fuzzing process, the reward probability distributions for all fuzzers tend to be relatively uniform, indicating an equal likelihood of reward for each strategy. This uniformity is particularly inevitabe in the early stage of the fuzzing process, where increasing the target program's code coverage is generally more straightforward. Consequently, the first few fuzzers selected might achieve significant coverage increases, inadvertently biasing the algorithm towards them and potentially overshadowing more effective fuzzers that are selected later.

% \wenxuan{fuzzing is random. an iteration shall be long enough to see the trend. we need batch.}
% Another challenge lies in the inherently random nature of fuzzing. Selecting a single strategy and executing one seed might not yield optimal performance. Moreover, in this condition, the selection process can be computationally expensive, making the overall system inefficient, especially when dealing with a large number of fuzzers.

% \wenxuan{an iteration can't be built on }
% Lastly, each strategy possesses a unique mutation energy, which reflects the number of mutations it can generate for a given seed. This variation in mutation energy means that comparing the performance of two different fuzzers based solely on the number of iterations they run may not provide an accurate assessment of their effectiveness. A fair comparison would allocate each strategy with a similar amount of resources to execute the fuzzing task each time it is selected.

% \wenxuan{code coverage is binary. reward is sparse. We need more information to guide TS to choose a better strategy, so we add a bonus of "cracking difficulty", which is evaluated by time}
% Lastly, reward based on code coverage is sparse.


% \subsection{Strategy Scheduling}
% \label{sec:selection}

% \begin{algorithm}[t]
%     \caption{\sys Strategy Scheduling}
%     \label{alg:fuzzer_selection}
%     \SetAlgoLined
%     \KwIn{A set of strategies $\mathcal{S}$, early stage time budget $T_E$, $max\_round, min\_round$, reset iteration interval $I_R$, iteration time budget $T_I$, stopping condition}
%     \textit{\textbf{Early Stage Starts}}\;
%     running time $t$ $\leftarrow$ 0\;
%      \While{$t < T_E$ }{
%       current strategy $ S \leftarrow$ RoundRobin($\mathcal{S}$)\;
%       $S.selections$ += 1 \;
%       $S$.run(), and return round time $t_r$\;
%       $t$ $\leftarrow$ $t$ + $t_r$\;
%       $S.total\_duration$ += $t_r$\;
%       }
%       \For{$S \in \mathcal{S}$}{
%         $S.avg\_round\_time$ $\leftarrow$ $ \text{floor} (\frac{S.total\_duration}{S.selections}$)\;
%         $S.Rounds \leftarrow \text{clip} (\frac{T_I}{S.avg\_round\_time}, max\_round, min\_round)$\;

%      }
%      \textit{\textbf{Main Stage Starts}}\;
%      iteration $i$ $\leftarrow$ 0\;
%      \While{stopping condition is not met}{
%         \If{i \% $I_R$ == 0}{
%             \For{$S \in \mathcal{S}$}{
%                 $S.\alpha_F$ $\leftarrow$ 1\;
%                 $S.\beta_F$ $\leftarrow$ 1\;
%             }
%         }
%         current fuzzer $ S \leftarrow$ ThompsonSampling($\mathcal{S}$)\;
%         \For{$round$=0, $round$<$S.Rounds$, $round$++}{
%             $S$.run(), and return round time $t_r$\;
%         }
     
%      }
% \end{algorithm}





% \begin{algorithm}[t]
%     \caption{Early Stage Scheduling}
%     \label{alg:early_stage}
%     \SetAlgoLined
%     \KwIn{A set of fuzzers $\mathcal{F}$, early stage time budget $T_E$, iteration time budget $T_I$, $max\_round, min\_round$}
%     running time $t$ $\leftarrow$ 0\;
%      \While{$t < T_E$ }{
%       current fuzzer $ F \leftarrow$ RoundRobin($\mathcal{F}$)\;
%       $F.selections$ += 1 \;
%       $F$.run(), and return round time $t_r$\;
%       $t$ $\leftarrow$ $t$ + $t_r$\;
%       $F.total\_duration$ += $t_r$\;
%       }
%       \For{$F \in \mathcal{F}$}{
%         $F.avg\_round\_time$ $\leftarrow$ $ \text{floor} (\frac{F.total\_duration}{F.selections}$)\;
%         $F.Rounds \leftarrow \text{clip} (\frac{T_I}{F.avg\_round\_time}, max\_round, min\_round)$\;

%      }
% \end{algorithm}

% \begin{algorithm}[t]
%     \caption{Main Stage Scheduling}
%     \label{alg:main_stage}
%     \SetAlgoLined
%     \KwIn{A set of fuzzers $\mathcal{F}$, iteration time budget $T_I$, reset iteration interval $I_R$, iteration time budget $T_I$, stopping condition}
%     iteration $i$ $\leftarrow$ 0\;
%      \While{stopping condition is not met}{
%         \If{i \% $I_R$ == 0}{
%             \For{$F \in \mathcal{F}$}{
%                 $F.\alpha_F$ $\leftarrow$ 1\;
%                 $F.\beta_F$ $\leftarrow$ 1\;
%             }
%         }
%         current fuzzer $ F \leftarrow$ ThompsonSampling($\mathcal{F}$)\;
%         \For{$round$=0, $round$<$F.Rounds$, $round$++}{
%             $F$.run(), and return round time $t_r$\;
%         }
     
%      }
% \end{algorithm}


% \subsection{Multi-Core Implementation}
% \label{sec:multi-core}

% In \autoref{alg:thompson_single}, we present the structure of the \sys framework. We first initialize the distributions for the probability of reward associated with each fuzzer (line 1). Then, in an iterative process, we employ the Thompson Sampling algorithm to select the most appropriate fuzzer for each run (line 3). The chosen fuzzer is then used to mutate input files (line 4), which are subsequently fed into the target program (line 7). 

% If the mutated input files trigger interesting results (increase the code coverage or crash the program), we add them to the set of interesting inputs. Finally, we evaluate the quality of the interesting inputs (line 12) and adjust the probability distribution of the reward for the employed fuzzer based on the evaluation results (line 13). We repeat this process until the stopping condition is met (line 2).


% In addition to the core functionalities of \sys, we introduce an innovative approach to assess the quality of the interesting inputs generated during the fuzzing process. This evaluation method is crucial, as it directly influences the rewards allocated to the selected fuzzer. The fundamental principle of our approach is that not all interesting inputs should be treated equally in the reward calculation.

% During the initial phases of fuzzing, a fuzzer may produce a significant number of inputs that increase the coverage of the target program. But soon, its coverage improvements cease: even after repeated mutation iterations, none of the mutated seeds it generates cover new code. In this case, the fuzzing process reaches a \textit{coverage stall}. In such scenarios, the fuzzer that successfully breaks through this coverage bottleneck deserves a higher reward. This breakthrough is pivotal, as it often leads to a subsequent surge in uncovering new interesting inputs, thereby rapidly expanding the program coverage.

% In contrast, the inputs discovered after this \textit{coverage stall}, despite contributing to coverage expansion, we may not assign a high reward to it. The rationale behind this reward mechanism is to prioritize the discovery of truly impactful inputs that can break through the bottleneck.


% To implement the proposed reward mechanism, for each mutant $m \in \mathcal{S}$, we record the execution index $E_m$ of the target program when $m$ is executed. Additionally, we record the minimum $E_{min}$ and maximum $E_{max}$ coverage increase intervals experienced by the target program, as well as $E_{last}$, the execution index for the most recent interesting input.

% \begin{algorithm}
%     \label{alg:evaluate}
%     \caption{Evaluate the Quality of the Interesting Inputs}
%     \SetAlgoLined
%     \KwIn{Interesting inputs set $\mathcal{S'}$, execution index $E$, minimum and maximum coverage increase interval $E_{min}$ and $E_{max}$, execution index $E_{last}$ for the last interesting input}
%     $r \leftarrow 0$\;
%     \For{mutant $m$ in $\mathcal{S'}$}{
%         interval $I$ $\leftarrow$ $E_m - E_{last}$\;
%         $E_{min} \leftarrow$ min($E_{min}$, $I$)\;
%         $E_{max} \leftarrow$ max($E_{max}$, $I$)\;
%         $r \leftarrow r + \frac{I - E_{min}}{E_{max} - E_{min}}$\;
%         $E_{last} \leftarrow E_m$
%     }
%     \KwOut{reward $r$}
% \end{algorithm}

% For each mutant $m$ contributing to an increase in the target program's coverage, we compute the interval $I$, defined as the difference between the execution index $E_m$ of the target program for $m$ and the execution index $E_{last}$ (line 3). Since the minimum and maximum intervals are not known in advance, we dynamically update them (lines 4-5). 

% Finally, we use Min-Max Normalization to calculate the individual reward $r$ for input $m$ (line 6), yielding values between 0 and 1. The larger the reward $r$ is, the better the quality of $m$ is. We sum up the reward $r$ for all interesting inputs in the set $\mathcal{S'}$ (line 2) and use it to quantify the selected fuzzer's contribution in this iteration.

% This reward mechanism prioritizes fuzzers that successfully overcome bottlenecks, awarding them higher rewards for breakthrough inputs. Conversely, during phases where coverage increases are more easily achieved, such as in the early stages or immediately following the \textbf{coverage stall}, the rewards are proportionally smaller. This approach incentivizes the generation of inputs that are critical in breaking through bottlenecks, thereby enhancing the overall effectiveness of the fuzzing process.

==> ccs/5-experiments-ccs.tex <==
\section{Experiment}
\label{sec:eval}

In this section, we comprehensively evaluate \sys to answer the following research questions (RQs):

\noindent{\bf RQ1.} \sys integrates a suite of advanced fuzzing tools, leveraging their combined strengths. 
When provided with identical computational resources, how does the collaborative fuzzing approach of \sys compare against the performance of the individual fuzzers it incorporates?

\noindent{\bf RQ2.} When compared to SOTA collaborative fuzzing method, \autofz, does \sys, enhanced with our proposed fuzzer evaluation and resource allocation method, demonstrate better performance?

\noindent{\bf RQ3.} \sys introduces three key techniques, including real-time synchronization via a global seed pool, fuzzer evaluation, and resource allocations. 
How do these key components individually contribute to the overall effectiveness of \sys?

\noindent{\bf RQ4.} How do key design (customized bandits) and hyper-parameters (time budget for each round $T_I$ and the
reset interval $I_R$) in our resource allocation method influence the overall performance metrics of \sys?


\subsection{Experiment Setup}
\label{subsec:exp_setup}

\noindent{\bf Environment setup.}
We conduct all experiments on two workstations, each equipped with an AMD EPYC 7763 64-core processor and 512GB of RAM. 
Within this setup, each fuzzer operates in a separate Docker container (note that \sys is considered a single fuzzer). 
The resource allocation for these containerized environments was deliberately constrained to a single CPU core and 2GB of shared memory, ensuring a standardized and controlled testing environment.

\noindent{\bf Configuration of \sys.}
% imperative -> necessary; designate -> specify; adequate -> appropriate
\sys performs periodic resets to adapt to changes in reward distributions. Also, \sys requires specifying an appropriate time budget for the fuzzer selected by the bandit algorithm. Unless specified otherwise, most of the experiments presented in this paper followed a configuration where the reset interval $I_R$ was established at 120 minutes, and a time budget $T_I$ of 120 seconds was allocated for each round.

\noindent{\bf Benchmark.}
% reputable -> popular; counteract -> mitigate;
Our evaluation leverages the fuzzing benchmarks provided by FuzzBench~\cite{metzman2021fuzzbench}, a popular source in the field.
Acknowledging the compatibility limitations of some existing fuzzers with FuzzBench, we also incorporated the Fuzzer Test Suite (FTS)~\cite{fuzzer_test_suite_2021} as an alternative benchmark. 
Each fuzzer, representing both our proposed solution and established fuzzing techniques, was subjected to a continuous testing period of 24 hours for every fuzzing target. To mitigate the inherent variability and ensure robust results, we executed each experiment 10 times, resulting in a cumulative computation time of 7.5 CPU years.

\noindent{\bf Metrics. }
% prevalent -> commonly used; gauging -> evaluating; designated -> specified; encompassed -> included
In line with the standard evaluation metrics typically used to assess fuzzing techniques, we chose branch coverage as the main criterion for evaluating the effectiveness of a fuzzer against a specific target program. As mentioned earlier, our evaluation covered a wide range of target programs from both FuzzBench and FTS. Considering the varying performance that different fuzzers show across different programs, we calculated the average score for each fuzzer to enable a more detailed and comparative analysis.

% nuanced -> /; disparities -> difference; holistic -> comprehensive
Average score is a concept introduced by FuzzBench~\cite{metzman2021fuzzbench} which serves as a benchmark for evaluating the overall performance of a fuzzer. This metric allows for a more balanced comparison by accounting for the performance difference across multiple target programs, thereby offering a comprehensive view of a fuzzer's effectiveness. 
More specifically, the fuzzer's score for each target equals dividing its median branch coverage by the maximum branch coverage recorded for that same target.
% Note that the highest relative performance does not necessarily correspond to 100\%.


\begin{table*}[t]
\caption{Fuzzer score summary in FuzzBench report. The fuzzers are organized based on average score, representing their average relative coverage. Those with higher values are positioned towards the left side of the table.
A green background signifies a superior score, whereas a blue background denotes the second-best score. Note that in FuzzBench report, any difference less than 1\% is considered as a random effect and thus disregarded. The symbol \dag \ indicates that the fuzzer encounters a crash before completing its 24-hour task. The symbol - indicates that the fuzzer does not support the target.}
\centering
\resizebox{1\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrr}
\toprule
Benchmark & \sys & AFL++ & honggfuzz & LAF-Intel & Radamsa & MOpt & AFL & AFLFast & FairFuzz  & DARWIN \\
\midrule
bloaty\_fuzz\_target & \cellcolor{lightgreen} 97.97 & \cellcolor{lightgreen} 97.41 & 77.56 & 96.38 & 82.45 & 94.95 & 93.65 & 93.78 & 80.52 & \dag 68.02 \\
curl\_curl\_fuzzer\_http & \cellcolor{lightgreen} 99.07 & \cellcolor{lightblue} 98.09 & 85.09 & 85.23 & 89.74 & 92.03 & 90.64 & 89.46 & 83.97 & \dag 62.99 \\
freetype2\_ftfuzzer & \cellcolor{lightgreen} 98.15 & \cellcolor{lightblue} 88.38 & 53.91 & 77.56 & 53.46 & 61.38 & 59.50 & 58.66 & 58.42 & \dag 21.27 \\
harfbuzz\_hb-shape-fuzzer & \cellcolor{lightgreen} 98.87 & \cellcolor{lightgreen} 98.84 & 81.73 & 97.22 & 84.47 & 96.42 & 95.74 & 95.34 & 88.69 & \dag 68.31 \\
jsoncpp\_jsoncpp\_fuzzer & \cellcolor{lightgreen} 100.00 & \cellcolor{lightgreen} 100.00 & \cellcolor{lightgreen} 100.00 & \cellcolor{lightgreen} 100.00 & \cellcolor{lightgreen} 100.00 & \cellcolor{lightgreen} 100.00 & \cellcolor{lightgreen} 100.00 & \cellcolor{lightgreen} 100.00 & \cellcolor{lightgreen} 100.00 & \cellcolor{lightgreen} 100.00 \\
lcms\_cms\_transform\_fuzzer & \cellcolor{lightgreen} 97.95 & \cellcolor{lightblue} 93.03 & 30.30 & 64.93 & 33.42 & 29.39 & 29.01 & 27.32 & 64.19 & 30.61 \\
libjpeg-turbo\_libjpeg\_turbo\_fuzzer & \cellcolor{lightgreen} 82.74 & \cellcolor{lightgreen} 82.65 & \cellcolor{lightgreen} 82.29 & \cellcolor{lightgreen} 82.65 & \cellcolor{lightgreen} 82.61 & \cellcolor{lightgreen} 82.26 & \cellcolor{lightgreen} 82.18 & \cellcolor{lightgreen} 82.19 & \cellcolor{lightgreen} 82.19 & \dag 81.64 \\
libpcap\_fuzz\_both & \cellcolor{lightgreen} 92.32 & \cellcolor{lightblue} 89.85 & 65.84 & 83.64 & 68.78 & 1.08 & 1.08 & 1.08 & 1.08 & \dag 0.00 \\
libpng\_libpng\_read\_fuzzer & \cellcolor{lightgreen} 95.95 & \cellcolor{lightgreen} 95.50 & 94.62 & \cellcolor{lightgreen} 95.52 & 92.47 & 93.07 & 93.02 & 92.12 & 93.19 & 93.26 \\
libxml2\_xml & \cellcolor{lightgreen} 99.61 & \cellcolor{lightgreen} 99.41 & 94.74 & - & 92.00 & 96.73 & 96.64 & 96.77 & 89.74 & 96.99 \\
libxslt\_xpath & \cellcolor{lightgreen} 98.31 & \cellcolor{lightgreen} 98.11 & 93.23 & 49.67 & 90.48 & 89.58 & 90.80 & 90.37 & 92.29 & 92.63 \\
mbedtls\_fuzz\_dtlsclient & \cellcolor{lightgreen} 74.73 & \cellcolor{lightgreen} 74.25 & 71.52 & 50.41 & 64.34 & 71.03 & 70.70 & 68.52 & 73.73 & \dag 49.30 \\
openh264\_decoder\_fuzzer & \cellcolor{lightgreen} 99.03 & 98.43 & 96.51 & \cellcolor{lightgreen} 99.28 & 79.75 & \cellcolor{lightgreen} 99.07 & \cellcolor{lightgreen} 99.06 & \cellcolor{lightgreen} 99.40 & 98.46 & \dag 0.00 \\
openssl\_x509 & \cellcolor{lightgreen} 99.95 & \cellcolor{lightgreen} 99.94 & 98.97 & \cellcolor{lightgreen} 99.59 & \cellcolor{lightgreen} 99.29 & \cellcolor{lightgreen} 99.69 & \cellcolor{lightgreen} 99.73 & \cellcolor{lightgreen} 99.72 & \cellcolor{lightgreen} 99.69 & \cellcolor{lightgreen} 99.91 \\
openthread\_ot-ip6-send-fuzzer & \cellcolor{lightblue} 77.05 & \cellcolor{lightgreen} 89.91 & 70.08 & 71.28 & 69.06 & 73.10 & 72.04 & 70.95 & 69.14 & \dag 0.00 \\
proj4\_proj\_crs\_to\_crs\_fuzzer & \cellcolor{lightgreen} 96.70 & \cellcolor{lightblue} 90.67 & 50.13 & 67.82 & 52.22 & 9.83 & 10.32 & 9.35 & 10.47 & \dag 0.70 \\
re2\_fuzzer & \cellcolor{lightgreen} 99.84 & \cellcolor{lightgreen} 99.43 & 98.39 & \cellcolor{lightgreen} 99.76 & 98.54 & 98.89 & \cellcolor{lightgreen} 99.34 & 98.63 & \cellcolor{lightgreen} 99.13 & \cellcolor{lightgreen} 99.01 \\
stb\_stbi\_read\_fuzzer & \cellcolor{lightgreen} 96.18 & \cellcolor{lightblue} 95.59 & 92.34 & 90.28 & 89.01 & 89.56 & 90.35 & 89.81 & 89.85 & 90.62 \\
systemd\_fuzz-link-parser & \cellcolor{lightgreen} 98.76 & \cellcolor{lightgreen} 98.35 & 88.64 & 97.93 & 89.67 & 90.91 & 90.50 & 90.70 & 84.30 & \dag 51.65 \\
vorbis\_decode\_fuzzer & \cellcolor{lightblue} 98.79 & \cellcolor{lightblue} 98.40 & 97.62 & \cellcolor{lightgreen} 99.38 & 93.75 & 97.58 & 97.74 & 97.70 & 97.54 & \dag 59.25 \\
woff2\_convert\_woff2ttf\_fuzzer & \cellcolor{lightblue} 98.56 & 97.36 & 89.19 & \cellcolor{lightgreen} 99.26 & 82.26 & 90.10 & 88.86 & 89.69 & 81.56 & \dag 62.95 \\
\hline
Median Score & \cellcolor{lightgreen} 98.31 & \cellcolor{lightblue} 97.41 & 88.64 & 90.28 & 84.47 & 90.91 & 90.64 & 90.37 & 84.30 & 62.99 \\
Average Score & \cellcolor{lightgreen} 95.26 & \cellcolor{lightblue} 94.46 & 81.56 & 81.32 & 80.37 & 78.89 & 78.61 & 78.17 & 78.01 & 58.53 \\
\bottomrule
\end{tabular}
}
\label{tab:fuzzbench}
\end{table*}

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=1.02\linewidth]{sources/figs/individual_small.pdf}
%     \vspace{-5mm}
%     \caption{Evaluation of \sys and individual fuzzers on FuzzBench: Each line plot in the graph represents the arithmetic mean along with a 95\% confidence interval, derived from 10 independent trials. ``Branch coverage'' denotes the count of branches that each fuzzer has explored.}
%     \label{fig:compare_individual}
%     \vspace{-2mm}
% \end{figure*}


\begin{table}[t]
\Large
\caption{The branch coverage of \sys vs. autofz-8 and full autofz. Each row displays the arithmetic mean and standard deviation of branch coverage for every fuzzer. The maximum branch coverage achieved for each target is also highlighted.}
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{l c c c c c c }
\toprule \multirow{2}{*}{ Benchmarks } & \multicolumn{2}{c}{ \sys-8 } & \multicolumn{2}{c}{ \autofz-8 } & \multicolumn{2}{c}{ \autofz } \\
\cline{2-7}
 & mean & std & mean & std & mean & std \\
\midrule
boringssl-2016-02-12 & 1671.7 & 0.48 & 1622.9 & 12.03 & \textbf{1678.5} & 17.06 \\
c-ares-CVE-2016-5180 & 42.9 & 0.32 & \textbf{43.0} & 0.00 & 42.9 & 0.32 \\
freetype2-2017 & \textbf{10946.4} & 418.56 & 7887.1 & 326.99 & 8236.8 & 234.77 \\
guetzli-2017-3-30 & \textbf{1409.9} & 3.75 & 1392.9 & 9.39 & 1399.6 & 8.25 \\
harfbuzz-1.3.2 & \textbf{4866.0} & 41.63 & 4622.8 &57.72 & 4722.3 &53.50 \\
json-2017-02-12 & 649.1 & 1.52 & 649.5 & 5.82 & \textbf{662.9} & 0.32 \\
libarchive-2017-01-04 & \textbf{5071.1} & 190.69 & 4453.0 & 308.46 & 4687.7 & 300.56 \\
libjpeg-turbo-07-2017 & \textbf{2028.9} & 91.89 & 1836.7 & 79.63 & 2026.6 & 42.24 \\
libpng-1.2.56 & 1054.1 & 9.54 & 1076.9 & 11.86 & \textbf{1090.0} & 8.82 \\
libssh-2017-1272 & \textbf{1068.0} & 59.60 & 1006.9 & 14.50 & 1064.9 & 54.02 \\
libxml2-v2.9.2 & \textbf{8308.8} & 292.49 & 3955.4 & 73.62 & 4406.6 & 353.30 \\
lcms-2017-03-21 & 1923.8 & 179.52 & \textbf{1991.8} & 39.44 & 1976.1 & 37.25 \\
openssl-1.0.1f & \textbf{5536.4} & 551.51 & 5058.8 & 822.06 & 5450.7 & 250.61 \\
openssl-1.0.2d & \textbf{2136.1} & 1.66 & 2126.4 & 3.37 & 2133.1 & 2.60 \\
openssl-1.1.0c-bignum & \textbf{2036.9} & 0.74 & 2034.8 & 0.42 & 2034.7 & 0.82 \\
openssl-1.1.0c-x509 & 6105.8 & 0.63 & 6144.0 & 3.62 & \textbf{6145.3} & 1.70 \\
openthread-2018-02-27-ip6 & 1412.5 & 318.97 & 1280.4 & 323.10 & \textbf{1412.8} & 320.93\\
openthread-2018-02-27-radio & 2783.7 & 240.00 & 2595.2 & 290.29 & \textbf{3260.8} & 42.63 \\
pcre2-10.00 & \textbf{9909.4} & 125.82 & 8956.5 & 73.64 & 9124.1 & 118.82 \\
proj4-2017-08-14 & 2461.4 & 192.53 & 1015.1 & 595.85 & \textbf{3568.7} & 43.01 \\
re2-2014-12-09 & \textbf{2485.3} & 7.10 & 2470.6 & 8.85 & 2478.7 & 7.24 \\
sqlite-2016-11-14 & \textbf{1981.0} & 1112.83 & 1551.5 & 147.60 & 1624.0 & 0.00 \\
vorbis-2017-12-11 & \textbf{1264.1} & 6.94 & 1236.3 & 10.75 & 1242.4 & 12.66 \\
woff2-2016-05-06 & 1071.9 & 23.32 & \textbf{1097.1} & 16.93 & 1062.7 & 33.05 \\
wpantund-2018-02-27 & \textbf{3315.2} & 99.03 & 3079.3 & 84.01 & 3176.1 & 52.75 \\
\midrule 
Average Coverage Enhancement & \multicolumn{2}{c}{-} & \multicolumn{2}{c}{16.0\%} & \multicolumn{2}{c}{4.8\%} \\
Average Score & \multicolumn{2}{c}{ 91.5 } & \multicolumn{2}{c}{ 84.3 } & \multicolumn{2}{c}{  89.6 }\\
\bottomrule
\end{tabular}}

\label{tab:autofz}
\end{table}

\subsection{Experiment Design}
\label{subsec:exp_design}
\noindent{\bf Experiment I.}
% 
To address RQ1, we isolated the fuzzers incorporated within \sys, treating them as individual fuzzers.
We then conducted experiments by operating \sys and each individual fuzzer against the targets from FuzzBench. %predetermined binaries from FuzzBench.
% juxtaposing -> compare
The experimental setup involved a 24-hour duration with every fuzzer deployed on identical computational resources. Then we conducted a comparative analysis of the branch coverage metrics, comparing the performance of \sys with that of the individual fuzzers.  We expect that \sys will have higher efficacy compared to the individual fuzzers, as \sys's bandit algorithm is adept at dynamically selecting the most efficient fuzzers over time.

\noindent{\bf Experiment II.}
% 
To address RQ2, we compare \sys with the state-of-the-art collaborative fuzzing framework. As is referenced in \autoref{subsec:bg_rw}, \autofz is recognized as the latest collaborative fuzzing framework, integrating a suite of 11 distinct fuzzers. In pursuit of addressing RQ2, we positioned \autofz as the baseline for comparison against \sys.

In our prior discussions, we established FuzzBench as the evaluation platform for \sys.
% Consequently, it seemed logical to employ FuzzBench for testing \autofz as well.
However, the implementation of \autofz is incompatible with FuzzBench, necessitating its evaluation on an alternate benchmark. It was also noted that despite both \autofz and \sys incorporating multiple fuzzers, the composition of these fuzzers is not identical, featuring unique elements such as Darwin in \sys and libFuzzer in \autofz.

% tailored -> changed
To facilitate an apple-to-apple, fair comparison, we changed the experimental design to operate on FTS, restricting the fuzzers to those mutually supported by both \autofz and \sys. This adjustment resulted in a revised toolkit comprising eight fuzzers (AFL, AFL++, AFLFast, LAF-Intel, MOpt, Radamsa, Angora, Fairfuzz) for both \autofz and \sys, henceforth referred to as \autofz-8 and \sys-8. 
Note that we enable \texttt{cmplog} within AFL++, a technique analogous to that utilized in RedQueen. \texttt{cmplog} is integrated as the default mode for AFL++ when conducting experiments on FuzzBench. This setup is applied in both Experiment I and Experiment II.
In this experiment, our primary focus was to compare the branch coverage between \autofz-8 and \sys-8.

% juxtapose -> compare; testament -> proof
We also compared \sys-8 with the complete setup of \autofz, which includes all 11 fuzzers. This comparison aimed to evaluate the unique features and strengths of \sys against a well-established benchmark in the field. Demonstrating that \sys-8 outperforms the fully equipped \autofz would further support the effectiveness of \sys. Showing that \sys-8 performs better than the fully equipped \autofz would further prove that \sys is more effective.

\noindent{\bf Experiment III.}
% 
To address the third research question (RQ3), we orchestrated an ablation study.

First, we configured \sys to operate without the utilization of a global seed pool. This allowed us to draw comparisons between a version of \sys that does not synchronize seeds among fuzzers and its standard configuration. In the absence of synchronization, there is a possibility for the fuzzers in \sys to redundantly traverse identical paths, potentially leading to a waste of time and resources. By observing alterations in performance within this setup, we can gain valuable insights into the importance of fuzzer synchronization in augmenting fuzzing efficiency.


% rudimentary -> simple
Second, we retained seed synchronization but altered \sys by substituting our bandit-based resource allocation mechanism with a simple random scheduling approach. Comparing the performance of this variant of \sys against the original \sys enabled us to quantify the impact of our bandit-based allocation mechanism on the efficacy of the fuzzing process.

It is important to underscore that both ablation experiments involved executing the original and modified versions of \sys against a quartet of carefully chosen target programs from FuzzBench. These programs—\texttt{bloaty}, \texttt{freetype2}, \texttt{woff2ttf}, and \texttt{lcms}—were selected for their diverse range in size and complexity, offering a representative spectrum of the challenges a fuzzer might encounter in navigating different code architectures.

To elaborate, \texttt{bloaty} is a large-scale program with 89,530 edges and is equipped with 94 seeds. Conversely, \texttt{freetype2} encompasses 19,056 edges but operates with a mere two seeds, representing a large program with a minimal seed count. On the other hand, \texttt{woff2ttf} is categorized as a smaller program with 10,923 edges, yet it is provisioned with 62 seeds. Lastly, \texttt{lcms}, the smallest in scale, incorporates 6,959 edges and operates with just one seed, illustrating a compact program with a sparse seed allocation.

\noindent{\bf Experiment IV.}
% 
To address the fourth research question (RQ4), we devised several alternative designs to substitute components within our system. By contrasting the performance of the original system against versions incorporating these alternative designs, we aim to elucidate the influence of specific design elements on the \sys's overall efficacy. Below, we detail the alternative designs we employed.

% rudimentary -> simple
To evaluate the impact of our proposed fuzzer assessment mechanism (outlined in \autoref{subsec:tech_measure}), we altered \autoref{alg:evaluate}. Specifically, we adjusted the reward allocation for fuzzer $F$ by incrementing $\alpha_F$ by 1 upon any new coverage discovery and increasing $\beta_F$ by 1 when it fails. Additionally, we deactivated the auto-cycle feature to facilitate precise reward calculation. These modifications culminated in a variant of \sys, integrating a simple fuzzer assessment approach.

Our exploration further extends to the implications of custom modifications to Thompson Sampling (TS) bandits within \sys. We modified \sys by eliminating the periodic resets inherent, while leaving the reward discretization unaltered. The reason behind preserving reward discretization lies in its fundamental role in ensuring the accurate functioning of TS bandits. Hence, \sys without periodic resets serves as a comparison variant in our study.

Beyond the specific customizations and fuzzer assessment, we recognized the potential significance of other variables, such as the time budget for each round $T_I$ and the reset interval $I_R$, in influencing overall fuzzing performance. In our investigation, we treat these parameters as hyperparameters akin to those in machine learning algorithms. Employing prevalent techniques for evaluating hyperparameter impacts on machine learning methodologies, we utilized the Nemenyi post-hoc test to determine if notable disparities exist across various configurations. Specifically, we adjusted $T_I$ between 90 to 180 seconds in 30-second increments and varied $I_R$ from 90 to 180 minutes at 30-minute intervals.



\subsection{Experiment Result}
\label{subsec:exp_result}


\noindent{\bf Experiment I.}% 
\autoref{tab:fuzzbench} shows the average score of each fuzzer across individual target programs after a 24-hour testing period. 
The table first shows that \sys achieves the highest median and average score across the FuzzBench targets.
Specifically, \sys outperforms all other individual fuzzers in 18 of the 21 evaluated targets.
This result validates \sys's capability in harnessing and ensembling the unique strengths of individual fuzzers. 
In other words, \sys's bandit algorithm is able to consistently allocate more resources to fuzzers with the best performance along the fuzzing process. 
As a result, it puts together an ensemble strategy with the best performance. 

In addition, we also observe that \sys is more stable than individual fuzzers. This is another advantage of being an ensemble strategy in that \sys can always choose a functional fuzzer and will not be largely affected by the failure of one or two fuzzers. 
The fuzzer management feature introduced in \autoref{subsec:impl_synchronization} also helps the stability. 
This feature enables \sys to promptly identify and address any issues with the fuzzers during operation, ensuring consistent performance.

However, it is noteworthy that despite its overall superior performance, \sys occasionally exhibits a slower initial growth in code coverage during the initial 30 to 60 minutes compared to certain individual fuzzers. We believe this is an expected characteristic of \sys's operation, as \sys necessitates multiple iterations to effectively explore and determine the dynamic effectiveness of the various fuzzers it includes.

Finally, we notice that the coverage of score of \sys demonstrates relatively marginal improvement than AFL++. 
This is mainly because AFL++ (with \textit{cmplog} enabled) performs much better than other fuzzers in most targets. By analyzing the seeds, we found that AFL++ dominates other fuzzers in code coverage. In the end, it's hard to see significant improvement.
However, we believe this does not dilute the necessity of \sys for the following reasons.
First, as demonstrated in~\autoref{sec:real-world-assessment}, \sys performs much better than the state-of-the-art fuzzers in mutation scores, a more reasonable metric for evaluating a fuzzer's ability to find vulnerabilities. 
Second, as an ensemble approach, \sys is more stable than individual fuzzers like AFL++.

% Replace autofz-11 with autofz (No need to come up with a new name)
% 
\noindent{\bf Experiment II.}
% 
\autoref{tab:autofz} presents a comparative analysis. The data reveal that \sys-8 outperforms \autofz-8 in 19 of the 25 evaluated programs, registering an average branch coverage enhancement of 16.0\%. This superior performance can be attributed primarily to \sys's robust seed synchronization approach and, more significantly, its bandits-based fuzzer scheduling strategy.

Moreover, \sys not only excels in comparison with \autofz-8 but also shows a competitive edge over the original \autofz configuration, which incorporates three additional fuzzers. Despite having fewer fuzzers, \sys-8 achieves an average branch coverage that exceeds that of the original \autofz by 4.8\%. This finding underscores the importance of bandit-based fuzzer scheduling, indicating that it can be more beneficial for fuzzing efficacy than the mere increase in the number of fuzzers within a collaborative framework.

It is also noteworthy that in instances where \sys-8 did not outperform \autofz-8, the decline in coverage was relatively marginal (not exceeding 3.5\%). The standard deviation of branch coverage for \sys-8 in these specific targets aligns closely with that of \autofz. Nevertheless, it is important to highlight an outlier occurrence, where \sys-8's standard deviation on the target \texttt{sqlite-2016-11-14} was exceptionally high, a result attributed to an isolated trial that yielded remarkably high branch coverage.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{sources/figs/ablation.pdf}
    \vspace{-5mm}
    \caption{Comparison among \sys and two variants. Each line plot represents the arithmetic mean along with a 95\% confidence interval, derived from 10 independent trials. The label \textit{random} refers to \sys that employs random resource allocation in each round, and \textit{no-sync} represents \sys operating without seed synchronization.}
    \label{fig:ablation_collaborative}
\end{figure}

\noindent{\bf Experiment III.}
% 
\autoref{fig:ablation_collaborative} delineates the performance differential between \sys and its derivative configurations. The ``random'' line illustrates \sys operating under a random resource allocation setup, whereas the ``no-sync'' line represents \sys devoid of a global seed pool, essentially operating without seed synchronization among fuzzers.

The graphical representation reveals a notable enhancement in \sys's performance when it incorporates a bandits-based resource allocation algorithm, registering a 22.0\% increment in branch coverage at the culmination of a 24-hour fuzzing campaign. This improvement is largely owed to the bandits-powered resource allocation strategy, which adeptly adapts to the immediate dynamics of fuzzing, thereby optimizing resource allocation and substantially augmenting fuzzing efficiency.

The comparison further illustrates that \sys, utilizing its synchronization mechanism, outperforms its non-synchronized counterpart by an average of 9.6\%. This enhancement in performance is primarily attributed to the real-time sharing of newly discovered insights among fuzzers, which promotes a more thorough and efficient exploration of the program space.

However, an exception is observed where fuzzers equipped with seed synchronization do not demonstrate superiority over their non-synchronized counterparts in the case of \texttt{woff2}. This deviation can be ascribed to the unique characteristics of the target - a sparse edge count combined with a plethora of seeds. In such circumstances, the advantage derived from inter-fuzzer knowledge exchange becomes less significant since each fuzzer already has considerable comprehension of the program's structure.


\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{sources/figs/ablation_ts.pdf}
    \vspace{-5mm}
    \caption{Comparison among \sys and two variants. Each line plot represents the arithmetic mean along with a 95\% confidence interval, derived from 10 independent trials. The label \textit{no-reset} refers to \sys without reset mechanism, and \textit{naive-reward} represents \sys adopting a naive algorithm to evaluate fuzzers.}
    \label{fig:ablation_ts}
\end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{sources/figs/sen_cd.pdf}
    \vspace{-3mm}
    \caption{Critical Difference (CD) among various configurations of \sys. The average ranking of fuzzers is represented by each number. The horizontal line indicates no critical difference in performance among the grouped fuzzers, as determined by the Nemenyi post-hoc test. Each label represents a variation of the depicted hyperparameter while keeping another parameter at its default values.}
    \label{fig:ablation_san_cd}
    \vspace{-3mm}
\end{figure}


\noindent{\bf Experiment IV.}
% 
\autoref{fig:ablation_ts} illustrates a comparative analysis between \sys and its variations. Notably, the variant termed \textit{naive-reward}, which employs a rudimentary method for fuzzer assessment, demonstrates a 5.8\% decline in branch coverage. The underlying reason is the simplistic nature of the naive fuzzer assessment mechanism, which updates the reward metrics solely based on discoveries by a fuzzer. This approach does not offer a nuanced evaluation of the relative complexity of each discovery, resulting in a less comprehensive assessment of fuzzer performance. 

In addition, as seen in~\autoref{fig:ablation_ts}, the \textit{no-reset} version of \sys, which excludes the reset operation during fuzzer evaluation, shows an 8.1\% decrease in branch coverage after the fuzzing campaign. The lack of a reset function hampers \sys's capability to counteract outdated information's impact, consequently undermining its ability to precisely adapt to changes in reward scenarios and efficiently utilize ongoing fuzzing activities' dynamics.

As discussed in~\autoref{subsec:exp_design}, the experiment also explores the sensitivity of \sys's configuration parameters, with the findings presented in~\autoref{fig:ablation_san_cd}. The Nemenyi post-hoc test results reveal no statistically significant differences among the configurations tested. This outcome suggests that \sys possesses robust adaptability, maintaining commendable performance across a spectrum of initial settings.


==> defs.tex <==
\usepackage{xparse}
\newcommand{\bnm}{\begin{newmath}}
\newcommand{\enm}{\end{newmath}}

\newcommand{\bea}{\begin{eqnarray*}}%
\newcommand{\eea}{\end{eqnarray*}}%

\newcommand{\bne}{\begin{newequation}}
\newcommand{\ene}{\end{newequation}}

\newcommand{\bal}{\begin{newalign}}
\newcommand{\eal}{\end{newalign}}

\newenvironment{newalign}{\begin{align}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{align}}

\newenvironment{newmath}{\begin{displaymath}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{displaymath}}

\newenvironment{neweqnarrays}{\begin{eqnarray*}%
\setlength{\abovedisplayskip}{-4pt}%
\setlength{\belowdisplayskip}{-4pt}%
\setlength{\abovedisplayshortskip}{-4pt}%
\setlength{\belowdisplayshortskip}{-4pt}%
\setlength{\jot}{-0.4in} }{\end{eqnarray*}}

\newenvironment{newequation}{\begin{equation}%
\setlength{\abovedisplayskip}{4pt}%
\setlength{\belowdisplayskip}{4pt}%
\setlength{\abovedisplayshortskip}{6pt}%
\setlength{\belowdisplayshortskip}{6pt} }{\end{equation}}


\newcounter{ctr}
\newcounter{savectr}
\newcounter{ectr}

\newenvironment{newitemize}{%
\begin{list}{\mbox{}\hspace{5pt}$\bullet$\hfill}{\labelwidth=15pt%
\labelsep=4pt \leftmargin=12pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{3pt} }}{\end{list}}


\newenvironment{newenum}{%
\begin{list}{{\rm (\arabic{ctr})}\hfill}{\usecounter{ctr} \labelwidth=17pt%
\labelsep=5pt \leftmargin=22pt \topsep=3pt%
\setlength{\listparindent}{\saveparindent}%
\setlength{\parsep}{\saveparskip}%
\setlength{\itemsep}{2pt} }}{\end{list}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Figure and table macros
%

\newcounter{mytable}
\def\mytable{\begin{centering}\refstepcounter{mytable}}
\def\endmytable{\end{centering}}

% \def\mytablecaption#1{\vspace{2mm}
%   \centerline{\textsf{Table \arabic{mytable}.~{#1}}}
%   \vspace{6mm}
%   \addcontentsline{lot}{table}{\protect\numberline{\arabic{mytable}}~{#1}}
% }


\newcounter{myfig}
\def\myfig{\begin{centering}\refstepcounter{myfig}}
\def\endmyfig{\end{centering}}

% \def\myfigcaption#1{
%              \vspace{2mm}
%              \centerline{\textsf{Figure \arabic{myfig}.~{#1}}}
%              \vspace{6mm}
%              \addcontentsline{lof}{figure}{\protect\numberline{\arabic{myfig}}~{#1}}}

\usepackage{caption}
\captionsetup{font=small, labelfont=bf}

\def\mytablecaption#1{\captionsetup{type=table}\caption*{\textsf{Table \arabic{mytable}.~{#1}}}}

\def\myfigcaption#1{\captionsetup{type=figure}\caption*{\textsf{Figure \arabic{myfig}.~{#1}}}}

\newlength{\saveparindent}
\setlength{\saveparindent}{\parindent}
\newlength{\saveparskip}
\setlength{\saveparskip}{\parskip}

\newcommand{\decOracle}{\textbf{Dec}}

\newcommand{\negsmidge}{{\hspace{-0.1ex}}}
\newcommand{\cdotsm}{\negsmidge\negsmidge\negsmidge\cdot\negsmidge\negsmidge\negsmidge}

\def\suchthatt{\: :\:}
\newcommand{\E}{{\rm I\kern-.3em E}}
\newcommand{\Prob}[1]{{\Pr\left[\,{#1}\,\right]}}
\newcommand{\Probb}[2]{{\Pr}_{#1}\left[\,{#2}\,\right]}
\newcommand{\CondProb}[2]{{\Pr}\left[\: #1\:\left|\right.\:#2\:\right]}
\newcommand{\CondProbb}[2]{\Pr[#1|#2]}
\newcommand{\ProbExp}[2]{{\Pr}\left[\: #1\:\suchthatt\:#2\:\right]}
\newcommand{\Ex}[1]{{\textnormal{E}\left[\,{#1}\,\right]}}
\newcommand{\Exx}{{\textnormal{E}}}
\newcommand{\given}{\ensuremath{\,\big|\,}}


\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\def\negl{\mathsf{negl}}


\newcommand{\secref}[1]{\mbox{Section~\ref{#1}}}
\newcommand{\appref}[1]{\mbox{Appendix~\ref{#1}}}
\newcommand{\thref}[1]{\mbox{Theorem~\ref{#1}}}
\newcommand{\defref}[1]{\mbox{Definition~\ref{#1}}}
\newcommand{\corref}[1]{\mbox{Corollary~\ref{#1}}}
\newcommand{\lemref}[1]{\mbox{Lemma~\ref{#1}}}
\newcommand{\clref}[1]{\mbox{Claim~\ref{#1}}}
\newcommand{\propref}[1]{\mbox{Proposition~\ref{#1}}}
\newcommand{\factref}[1]{\mbox{Fact~\ref{#1}}}
\newcommand{\remref}[1]{\mbox{Remark~\ref{#1}}}
\newcommand{\figref}[1]{\mbox{Figure~\ref{#1}}}
% \renewcommand{\algref}[1]{\mbox{Algorithm~\ref{#1}}}
% \newcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
% Have to use \renewcommand because exists already in amsmath
\renewcommand{\eqref}[1]{\mbox{Equation~(\ref{#1})}}
\newcommand{\consref}[1]{\mbox{Construction~\ref{#1}}}
\newcommand{\tabref}[1]{\mbox{Table~\ref{#1}}}

\newcommand{\get}{{\:{\leftarrow}\:}}
\newcommand{\gett}[1]{\:{\leftarrow}_{#1}\:}
\newcommand{\getsr}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle\$$}}}\:}}
\newcommand{\getm}{{\:\leftarrow_{\mdist}\:}}
\newcommand{\getd}{{\:\leftarrow_{\ddist}\:}}
%\newcommand{\getm}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \mdist$}}}\:}}
\newcommand{\getk}{{\:\leftarrow_{\kdist}\:}}
%\newcommand{\getk}{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle \kdist$}}}\:}}
\newcommand{\getp}{{\:\leftarrow_{p}\:}}



\newcommand{\gamesfontsize}{\small}
\newcommand{\fpage}[2]{\framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}}
\newcommand{\mpage}[2]{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize  #2 \end{minipage}}

\newcommand{\hpages}[3]{\begin{tabular}{cc}\begin{minipage}[t]{#1\textwidth} #2 \end{minipage} & \begin{minipage}[t]{#1\textwidth} #3 \end{minipage}\end{tabular}}

\newcommand{\hpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #3 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #4 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #4 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #6 \end{minipage}
        \end{tabular}
    }

\newcommand{\hpagessss}[8]{
        \begin{tabular}{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \begin{minipage}[t]{#1\textwidth}\gamesfontsize #5 \end{minipage}
        &
        \begin{minipage}[t]{#2\textwidth}\gamesfontsize #6 \end{minipage}
        &
        \begin{minipage}[t]{#3\textwidth}\gamesfontsize #7 \end{minipage}
        &
        \begin{minipage}[t]{#4\textwidth}\gamesfontsize #8 \end{minipage}
        \end{tabular}
    }


\newcommand{\hfpages}[3]{\hfpagess{#1}{#1}{#2}{#3}}
\newcommand{\hfpagess}[4]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #3 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagesss}[6]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #4 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        \end{tabular}
    }
\newcommand{\hfpagessss}[8]{
        \begin{tabular}[t]{c@{\hspace*{.5em}}c@{\hspace*{.5em}}c@{\hspace*{.5em}}c}
        \framebox{\begin{minipage}[t]{#1\textwidth}\setstretch{1.1}\gamesfontsize #5 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#2\textwidth}\setstretch{1.1}\gamesfontsize #6 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#3\textwidth}\setstretch{1.1}\gamesfontsize #7 \end{minipage}}
        &
        \framebox{\begin{minipage}[t]{#4\textwidth}\setstretch{1.1}\gamesfontsize #8 \end{minipage}}
        \end{tabular}
    }

\newcommand{\vecw}{\mathbf{w}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\load}{L}
\newcommand{\coll}{\mathsf{Coll}}
\newcommand{\nocoll}{\overline{\mathsf{Coll}}}


\newcommand{\Img}{\textsf{Img}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Fonts and symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\funcfont{\textsf}
\newcommand\variablefont{\texttt}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW COMMANDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def \Perm {\funcfont{Perm}}
\def \calC {{\mathcal{C}}}
\def \calU {{\mathcal{U}}}
\renewcommand{\u}{\ensuremath{u}}
\newcommand{\unew}{\ensuremath{\tilde{u}}}

\newcommand{\calN}{\mathcal{N}}
\def \sspace {{\mathcal{S}}}
\def \strings {{\mathcal{S}}}
\def \slen {{s}}
\def \kspace {{\mathcal{K}}}
\def \kspacesize {{m}}
\def \mspacesize {{n}}
\def \kdict {D}
\def \dictsize {d}
\newcommand{\kdist}{p_k}
\newcommand{\mdist}{\ensuremath{{W}}}
\newcommand{\alldist}{\rho}
\newcommand{\pwdist}{\transgen}
\newcommand{\ddist}{\rho_{dec}}
\newcommand{\PWset}{{\mathcal{P}}}  % TODO: fix, same as \pwdist
\newcommand{\PWsetvec}{\vec{\mathcal{P}}}
\newcommand{\PWvec}{\vec{P}}
\newcommand{\domvec}{\vec{D}}
\newcommand{\humanornot}{\vec{h}}
\newcommand{\dom}{\textsf{dom}}
%\def \kdist {{\kappa}}
%\def \mdist {{\mu}}
%\def \ddist {{\delta}}
\def \pspace {{\mathcal{P}}}
\def \mpspace {{\mathcal{MP}}}
\def \cspace {{\mathcal{C}}}
\def \key {\kappa}
\def \msg {M}
\def \seed {S}
\def \ctxt {C}
\def \ctxtpart {C_2}
\newcommand{\genprime}{{\textsf{GenPrime}}}
\newcommand{\isprime}{{\textsf{IsPrime}}}
\newcommand{\LeastLesserPrime}{{\textsf{PrevPrime}}}
\newcommand{\pwset}{\mathcal{S}}
\newcommand{\DTE}{{\textsf{DTE}}}
\newcommand{\encode}{{\textsf{encode}}}
\newcommand{\decode}{{\textsf{decode}}}

\newcommand{\DTEsingle}{{\textsf{1PW-DTE}}}
\newcommand{\encodesingle}{{\textsf{1PW-encode}}}
\newcommand{\decodesingle}{{\textsf{1PW-decode}}}

\newcommand{\DTErss}{{\textsf{RSS-DTE}}}
\newcommand{\encoderss}{{\textsf{RSS-encode}}}
\newcommand{\decoderss}{{\textsf{RSS-decode}}}

\newcommand{\DTEindep}{{\textsf{MPW-DTE}}}
\newcommand{\encodeindep}{{\textsf{MPW-encode}}}
\newcommand{\decodeindep}{{\textsf{MPW-decode}}}


\newcommand{\DTEsub}{{\textsf{SG-DTE}}}
\newcommand{\encodesub}{{\textsf{SG-encode}}}
\newcommand{\decodesub}{{\textsf{SG-decode}}}
\newcommand{\decodekamf}{{\textsf{KAMF-decode}}}
\newcommand{\DTEis}{{\textsf{IS-DTE}}}
\newcommand{\encodeis}{{\textsf{is-encode}}}
\newcommand{\decodeis}{{\textsf{is-decode}}}
\newcommand{\DTErej}{{\textsf{REJ-DTE}}}
\newcommand{\encoderej}{{\textsf{rej-encode}}}
\newcommand{\decoderej}{{\textsf{rej-decode}}}
\newcommand{\DTErsarej}{{\textsf{RSA-REJ-DTE}}}
\newcommand{\encodeRSAREJ}{{\textsf{rsa-rej-encode}}}
\newcommand{\decodeRSAREJ}{{\textsf{rsa-rej-decode}}}
\newcommand{\DTErsainc}{{\textsf{RSA-INC-DTE}}}
\newcommand{\encodeRSAINC}{{\textsf{rsa-inc-encode}}}
\newcommand{\decodeRSAINC}{{\textsf{rsa-inc-decode}}}
\newcommand{\DTEunf}{{\textsf{UNF-DTE}}}
\newcommand{\DTEnunf}{{\textsf{NUNF-DTE}}}


%\newcommand{\encodeis}{{\textsf{encode}_{\textrm{is}}}}
%\newcommand{\decodeis}{{\textsf{decode}_{\textrm{is}}}}
\newcommand{\rep}{\textsf{rep}}
\newcommand{\isErr}{\epsilon_{\textnormal{is}}}
\newcommand{\incErr}{\epsilon_{\textnormal{inc}}}
\def \enc {{\textsf{E}}}
\def \dec {{\textsf{D}}}
\def \SEscheme {{\textsf{SE}}}
\def \HEscheme {{\textsf{HE}}}
\def \CTR {{\textsf{CTR}}}
\def \encHE {{\textsf{HEnc}}}
\def \HIDE {{\textsf{HiaL}}}
\def \encHIDE {{\textsf{HEnc}}}
\def \decHIDE {{\textsf{HDec}}}
\def \decHE {{\textsf{HDec}}}
\def \encHEt {{\textsf{HEnc2}}}
\def \decHEt {{\textsf{HDec2}}}

\newcommand{\myind}{\hspace*{1em}}
\newcommand{\thh}{^{\textit{th}}} % th
\newcommand{\concat}{\,\|\,}
\newcommand{\dotdot}{..}
\newcommand{\emptystr}{\varepsilon}

\newcommand{\round}{\textsf{round}}

\newcommand{\alphabar}{\overline{\alpha}}
\newcommand{\numbinsbar}{\overline{b}}
\newcommand{\numballs}{a}
\newcommand{\numbins}{b}

%\def \encHE {{\sf{enc}^{HE}}}
%\def \decHE {{\sf{dec}^{HE}}}
%\def \encHEt {{\sf{enc}^{HE2}}}
%\def \decHEt {{\sf{dec}^{HE2}}}
\def \idealHE {{\mathcal{HE}}}
\def \IEnc {{\mathbf{\rho}}}
\def \IDec {{\mathbf{\rho^{-1}}}}
\def \OEnc {{\mathbf{Enc}}}
\def \ODec {{\mathbf{Dec}}}
\newcommand{\SimuProc}{\mathbf{Sim}}
\newcommand{\ROProc}{\mathbf{RO}}
\newcommand{\PrimProc}{\mathbf{Prim}}
\def \stm {g}
\def \istm {\hat{g}}
\def \kts {{f}}
\def \lex {{\sf lex}}
\def \part {part}
\def \kd {{\sf{kd}}}
\def \msgdist {{d}}
\def \keydist {{r}}
\def \ind {{\sf{index}}}
\def \kprf {z}
\def \adv {{\mathcal A}}
\def \pwds {u}
\newcommand{\mpw}{mpw}
\newcommand{\pw}{w}
\newcommand{\pwvec}{\vec{\pw}}
\newcommand{\vecx}{\vec{x}}
\def \tokens {v}
\def \calP{{\mathcal{P}}}
\def \template{{\mathcal{T}}}
\def \vaultset{{\mathcal{V}}}
\def \ext {{\sf ext}}
\def \offset {\delta}
\def \maxweight {\epsilon}
\def \advo {{\mathcal{A}}^{*}}

\newcommand{\Chall}{\textsf{Ch}}
\newcommand{\Test}{\textnormal{\textsf{Test}}}
\newcommand{\RoR}{\textsf{RoR}}
\newcommand{\MI}{\textnormal{MI}}
\providecommand{\MR}{\textnormal{MR}}
\newcommand{\MRCCA}{\textnormal{MR-CCA}}
\newcommand{\SAMP}{\textnormal{SAMP}}
\newcommand{\DTEgame}{\textnormal{SAMP}}
\newcommand{\KR}{\textnormal{KR}}
\newcommand{\advA}{{\mathcal{A}}}
\newcommand{\advR}{{\mathcal{R}}}
\newcommand{\advB}{{\mathcal{B}}} % 
\newcommand{\advC}{{\mathcal{C}}} % C
\newcommand{\advD}{{\mathcal{D}}} % D
\newcommand{\advE}{{\mathcal{E}}}
\newcommand{\advF}{{\mathcal{F}}}
\newcommand{\advG}{{\mathcal{G}}}
\newcommand{\advI}{{\mathcal{I}}}
\newcommand{\nextval}{\;;\;}
\newcommand{\TabC}{\texttt{C}}
\newcommand{\TabR}{\texttt{R}}
\newcommand{\Hash}{H}
\newcommand{\Cipher}{\pi}
\newcommand{\CipherInv}{\pi^{-1}}
\newcommand{\simu}{{\mathcal S}}
\newcommand{\prim}{P}
\newcommand{\maxguess}{\gamma}


\newcommand{\bigO}{\mathcal{O}}
\newcommand{\calG}{{\mathcal{G}}}

\def\sqed{{\hspace{5pt}\rule[-1pt]{3pt}{9pt}}}
\def\qedsym{\hspace{2pt}\rule[-1pt]{3pt}{9pt}}

\newcommand{\Colon}{{\::\;}}
\newcommand{\good}{\textsf{Good}}

\newcommand\Tvsp{\rule{0pt}{2.6ex}}
\newcommand\Bvsp{\rule[-1.2ex]{0pt}{0pt}}
\newcommand{\TabPad}{\hspace*{5pt}}
\newcommand\TabSep{@{\hspace{5pt}}|@{\hspace{5pt}}}
\newcommand\TabSepLeft{|@{\hspace{5pt}}}
\newcommand\TabSepRight{@{\hspace{5pt}}|}


\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}
\newcommand{\comma}{\textnormal{,}}

\renewcommand{\paragraph}[1]{\vspace*{6pt}\noindent\textbf{#1}\;}

\newcommand{\weirvault}{\textsf{Pastebin}\xspace}
\newcommand{\ndssvault}{\textsf{DBCBW}\xspace}




\newcommand{\reminder}[1]{ [[[ \marginpar{\mbox{$<==$}} #1 ]]] }

%
% New theorem types: (Already in CCS template)
%
\newtheorem{observation}{Observation}
%\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{fact}{Fact}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{proposition}{Proposition}
% \newtheorem{example}{Example}

%
% Definitions:
%
\def \blackslug{\hbox{\hskip 1pt \vrule width 4pt height 8pt
    depth 1.5pt \hskip 1pt}}
\def \qed{\quad\blackslug\lower 8.5pt\null\par}
% In-line QED, for ending a proof with a $$ formula
% In-line QED, for ending a proof with a $$ formula
\def \inQED{\quad\quad\blackslug}
\def \Qed{\QED}
\def \QUAD{$\Box$}
\def \Proof{\par\noindent{\bf Proof:~}}
\def \proof{\Proof}
\def \poly {\mbox{$\mathsf{poly}$}}
\def \binary {\mbox{$\mathsf{binary}$}}
\def \ones {\mbox{$\mathsf{ones}$}}
\def \rank {\mbox{$\mathsf{rank}$}}
\def \bits {\mbox{$\mathsf{bits}$}}
\def \factorial {\mbox{$\mathsf{factorial}$}}
\def \fr {\mbox{$\mathsf{fr}$}}
\def \pr {\mbox{$\mathsf{pr}$}}
\def \zon {\{0,1\}^n}
\def \zo  {\{0,1\}}
\def \zok {\{0,1\}^k}
\def \mo {s}


\def\utilcnt{\ensuremath{\mu_{\mathrm{cnt}}}}
\def\utiltime{\ensuremath{\mu_{\mathrm{time}}}}
\def\ex{\ensuremath{{\mathrm{ex}}}}
\def\rlx{\ensuremath{{\mathrm{rlx}}}}
\def\tp{\textsf{TP}}
\def\cp{\textnormal{\textsf{CP}}\xspace}
\def\edistcutoff{\edist}
\def\entcutoff{\ensuremath{m}}
\def\relentcutoff{{\sigma}}
\def\mutt{\mu_{\mathrm{tt}}}

\newcommand{\Hdot}{H(\mbox{ } \cdot \mbox{ }  , \mbox{ } \del)}


\newcounter{mynote}[section]
\newcommand{\notecolor}{blue}
\newcommand{\thenote}{\thesection.\arabic{mynote}}
\newcommand{\tnote}[1]{\refstepcounter{mynote}{\bf \textcolor{\notecolor}{$\ll$TomR~\thenote: {\sf #1}$\gg$}}}

\newcommand{\fixme}[1]{{\textcolor{red}{[FIXME: #1]}}}
\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}


\newcommand\ignore[1]{}


\newcommand\simplescheme{simple}


\newcommand{\KDF}{\mathsf{KDF}}
\newcommand{\salt}{\mathsf{sa}}
\newcommand{\PRF}{F}
\newcommand{\subgram}{\mathsf{SG}}
\newcommand{\popdomains}{\mathcal{D}}

\newcommand{\retrieve}{\textsf{Sync}}
\newcommand{\update}{\textsf{Insert}}

\newcommand{\dictW}{\textbf{D1}\xspace}
\newcommand{\dictF}{\textbf{D2}\xspace}

\newcommand{\str}{\text{str}}
\newcommand{\calS}{{\mathcal S}}

% \newcommand{\new}[1]{\textcolor{red}{\sf #1}}
\newcommand{\new}[1]{#1}


%% ------------------------- Rahul -----------------------
\newcounter{rcnote}[section]
\newcommand{\rcthenote}{\thesection.\arabic{rcnote}}
\newcommand{\rcnote}[1]{\refstepcounter{rcnote}{\bf \textcolor{magenta}{$\ll$RC~\rcthenote: {\sf #1}$\gg$}}}

\newcounter{mrnote}[section]
\newcommand{\mrthenote}{\thesection.\arabic{mrnote}}
\newcommand{\mrnote}[1]{\refstepcounter{mrnote}{\bf \textcolor{green}{$\ll$MR~\mrthenote: {\sf #1}$\gg$}}}

\newcounter{fknote}[section]
\newcommand{\fkthenote}{\thesection.\arabic{fknote}}
\newcommand{\fknote}[1]{\refstepcounter{fknote}{\bf \textcolor{blue}{$\ll$FK~\fkthenote: {\sf #1}$\gg$}}}

\newcounter{anote}[section]
\newcommand{\ajthenote}{\thesection.\arabic{anote}}
\newcommand{\anote}[1]{\refstepcounter{anote}{\bf \textcolor{cyan}{$\ll$AJ~\ajthenote: {\sf #1}$\gg$}}}



\newcommand{\mytab}{\hspace*{.4cm}}
\def\half{{1\over 2}}
\newcommand{\NT}[1]{\texttt{#1}}
\DeclareMathSymbol{\mlq}{\mathord}{operators}{``}
\DeclareMathSymbol{\mrq}{\mathord}{operators}{`'}
\newcommand{\calO}{{\mathcal O}}
\newcommand{\calA}{{\mathcal A}}
\newcommand{\kamfplus}{Kamouflage\textbf{+}\xspace}
% \newcommand{\genfrom}[1]{\;{\stackrel{\,#1}{\leftarrow}}\;}
\newcommand{\genfrom}[1]{{\:{\leftarrow{\hspace*{-3pt}\raisebox{.75pt}{$\scriptscriptstyle#1$}}}\:}}
%\newcommand{\genfrom}[1]{\;\leftarrow{\tiny \$} #1\;}
\newcommand{\twopartdef}[4]
{
  \left\{
    \begin{array}{ll}
      #1 & \mbox{if } #2 \\[4pt]
      #3 & #4
      \end{array}
      \right.
}
\newcommand{\threepartdef}[6]
{
  \left\{
    \begin{array}{lll}
      #1 & \mbox{if } #2 \\
      #3 & \mbox{if } #4 \\
      #5 & \mbox{if } #6
      \end{array}
      \right.
}

\newcommand{\gt}[1]{\gamma_{#1,\maxdist}}
\newcommand{\gmt}[2]{\gamma_{#1,#2}}
\def\nh{\ensuremath{N}}
\def\ball{\ensuremath{B}}
\def\anh{\ensuremath{\tilde{N}_k}}
% \newcommand{\nh}[2]{{N_{#1}(#2)}}

\newcommand{\ballsizet}[1]{{\beta_{#1,\maxdist}}}
\newcommand{\ballsize}[2]{{\beta_{#1,#2}}}
\newcommand{\rh}[2]{{\bf R}_{#1, #2}}
\newcommand{\rhf}[2]{R_{f, \gamma}}
\newcommand{\realm}{{m}}
% \newcommand{\inputm}{{\tilde{m}}}
\newcommand{\lmid}{\ell_{\realm, m'}}
\newcommand{\cipherlength}{n}
\renewcommand{\SS}{\textsf{SS}}
\newcommand{\Rec}{\textsf{Rec}\xspace}
\newcommand{\rec}{\textsf{rec}\xspace}
\newcommand{\Rep}{\textsf{Rep}\xspace}
\newcommand{\Gen}{\textsf{Gen}}
\newcommand{\dis}{\textsf{dis}}

\def\chk{\textnormal{\textsf{Chk}}\xspace}
\def\reg{\textnormal{\textsf{Reg}}\xspace}
\def\exchk{\textnormal{\textsf{ExChk}}\xspace}
\def\adpchk{\textnormal{\textsf{AdpChk}}\xspace}
\def\RKROR{\textnormal{MKROR}\xspace}
\def\SRKROR{\textnormal{SKROR}\xspace}
\def\ROR{\textnormal{ROR}\xspace}
\def\ROBUST{\textnormal{ROB}\xspace}
\def\OFFDIST{\textnormal{OFFDIST}\xspace}
\def\POFFDIST{\overline{\textnormal{OFFDIST}}\xspace}
\def\OFFGUESS{\textnormal{OFFGUESS}\xspace}
\def\ONGUESS{\overline{\textnormal{ONGUESS}}\xspace}
\def\ONATTACK{\textnormal{ONATTACK}\xspace}
\def\adp{\ensuremath{\Pi\xspace}}
\def\Check{\textnormal{\textsf{Checker}}}
\def\CheckPtxt{\textnormal{\textsf{PChecker}}}
\def\trans{\textnormal{\ensuremath{T}}}
\def\transgen{\textnormal{\ensuremath{\mathcal{T}}}}
\def\pke{\ensuremath{\mathcal{E}}}
\def\pkenc{\ensuremath{\pke^{\mathrm{enc}}}}
\def\pkdec{\ensuremath{\pke^{\mathrm{dec}}}}
\def\sH{\ensuremath\mathrm{H}^s}
\def\H{\ensuremath{\mathsf{H}}\xspace}
\def\T{\ensuremath{\mathsf{T}}\xspace}
\def\W{\ensuremath{\mathsf{W}}\xspace}
\def\F{\ensuremath{\mathsf{F}}\xspace}
\def\ret{\ensuremath{\mathrm{return}}\xspace}
\def\cs{\ensuremath{t}} % Cache Size
\def\waitlen{\ensuremath{\omega}\xspace} %waitlist size
\newcommand{\M}{{\mathcal{M}}}
\newcommand{\ent}{{\bf H}}
\newcommand{\Hfuzzy}{{\mathrm{H}}^{\rm fuzz}}
\newcommand{\Hminfuzzy}{{\mathrm{H}}^{{\rm{fuzz}}}_{t,\infty}}
\newcommand{\Hpfuzzy}{{\mathrm{H}}^{{\rm{pfuzz}}}}
\newcommand{\Hinf}{{\bf H}^{{\rm \min}}_{\infty}}
\newcommand{\Hminpfuzzy}{{\bf H}^{{\rm pfuzz}}_{t,\infty}}


\def\sa{{\sf sa}}
\def\err{{\varepsilon}}%^{(e)}}}
\newcommand{\dist}{\mathcmd{p}}
\newcommand{\distest}{\hat{\mathcmd{p}}}
\newcommand{\distvec}{\mathbf{\dist}}
\newcommand{\distvecest}{\hat{\mathbf{p}}}
\newcommand{\w}{{w}}
\newcommand{\wnew}{\tilde{w}}
\newcommand{\m}{{w}}
\newcommand{\mnew}{{\tilde{m}}}
\newcommand{\mspacevec}{\mathcmd{\mathbf{W}}}
\newcommand{\mvec}{\mathcmd{\mathbf{\m}}}
\newcommand{\mvecss}[1]{\mvec_1\ldots\mvec_{#1}}
\renewcommand{\mspace}{\mathcmd{W}}
\newcommand{\mspacebot}{{\mspace}_\bot}

\newcommand{\similar}{\mathrm{sim}}
\newcommand{\similarvec}{\mathrm{\mathbf{sim}}}

\def \mvecnew{{\tilde{\mvec}}}
\newcommand{\mvecnewss}[1]{\mvecnew_1\ldots\mvecnew_{#1}}

\DeclareDocumentCommand{\edist}{o o}{
  \ensuremath{
    \IfNoValueTF{#1}{{d}}{{\sf d}(#1,#2)}
  }
}

\newcommand{\utilinc}{\mu}
\newcommand{\secloss}{\Delta}
\newcommand{\seclossg}{\Delta^\textnormal{greedy}}
\newcommand{\seclosso}{\Delta}
%\newcommand{\maxlambda}{\lambda^*}
%\newcommand{\maxfuzzlambda}{\tilde{\lambda}^*}
\newcommand{\fuzzlambda}{\lambda^\textnormal{fuzzy}}
\newcommand{\greedylambda}{\lambda^\textnormal{greedy}}
\newcommand{\greedylambdaon}{\tilde{\lambda}^\mathrm{on}}
\newcommand{\greedylambdaoff}{\tilde{\lambda}^\mathrm{off}}
\newcommand{\seclosson}{\secloss^\mathrm{on}}
\newcommand{\seclossoff}{\secloss^\mathrm{off}}
\def \edit {\ensuremath{e}}
\newcommand\error{e}
\newcommand\tab[1][1cm]{\hspace*{#1}}

\newcommand{\mathcmd}[1]{\ensuremath{#1}\xspace} % to use a command both in math mode and non-math mode
\newcommand{\minentropy}[1]{\ensuremath{\operatorname{H_\infty}\olrk{#1}}}
\newcommand{\fuzzyminentropy}[1]{\ensuremath{\operatorname{H^{fuzz}_{\maxdist, \infty}}\olrk{#1}}}
\providecommand{\condminentropy}[2]{\ensuremath{\operatorname{\tilde{H}_\infty}\olrk{#1|#2}}}
\newcommand{\s}{\mathcmd{s}}
\newcommand{\typo}{\mathcmd{\tilde{\m}}}
\newcommand{\typoj}[1]{\ensuremath{(\typo_{#1}, j_{#1})}}
\newcommand\typojprime[1]{{(\typo_{#1}, j'_{#1})}}
\renewcommand\contrib[2]{\mathsf{cont}\left[{#1}/{#2}\right]}
\def\typovec{\ensuremath{\{\typo_i\}_{i=1}}}
\def\opttypovec{\ensuremath{\{\typo^*_i\}_{i=1}}}
\def\slotguess{\textsf{SlotGuess}}
\def\typodist{\ensuremath{\tau_\pw}}
\def\cachedtypodist{\ensuremath{{\tilde{\tau}}_{\pw}}}
\def\typodistest{\ensuremath{{\hat{\tau}}_{\pw}}}
\def\incache{T_\pw}
\newcommand{\fuzzylambda}{\ensuremath{\lambda^{\mathrm{fuzzy}}}}
%\newcommand{\errorprob}[2]{\mathcmd{\tau_{#1}({#2})}}
\newcommand{\errordist}{\mathcmd{\tau}}
\newcommand{\famdist}{\mathcmd{\mathcal{W}}}
\def\guessw{\ensuremath{W}}
\newcommand{\precdist}{W}
\newcommand{\entdef}{Z}
\newcommand{\PW}{\mathcmd{\mathcal{W}}}
\newcommand{\cachedom}{\mathcmd{\mathcal{S}}}
\newcommand{\supp}{\mbox{supp}}
\newcommand{\olrk}[1]{\ifx\nursymbol#1\else\!\!\mskip4.5mu plus 0.5mu\left(\mskip0.5mu plus0.5mu #1\mskip1.5mu plus0.5mu \right)\fi}

\newcommand{\errorprob}[1]{\mathcmd{\tau_{#1}}}
\newcommand{\errorpr}[2]{\mathcmd{\errorprob{#1}{(#2)}}}
\newcommand{\Expectation}{\mathop{\mathbb E}}
\newcommand{\hash}[2]{\mathcmd{F(#1, #2)}}
\newcommand{\hashj}[3]{\mathcmd{F_{#3}(#1, #2)}}
\newcommand{\rhh}{\mathcmd{y}}
\newcommand{\x}{\mathcmd{x}}
\newcommand{\range}{\mathcmd{R}}
\newcommand{\lmm}{\mathcmd{l_\w}}
\newcommand{\rmm}{\mathcmd{r_\w}}
\newcommand{\conflict}[2]{\mathcmd{C_{#1, #2}}}
\newcommand{\Probsub}[2]{{\Pr_{#1}\left[\,{#2}\,\right]}}
\newcommand{\Condprobsub}[3]{{\Pr}_{#1}\left[\: #2\:\left|\right.\:#3\:\right]}
\newcommand{\wmid}{l_{\w, \w^\prime}}
\newcommand{\realhash}{\mathcmd{z}}
\newcommand{\collhash}{\mathcmd{z^\prime}}
\newcommand{\floor}[1]{\left \lfloor #1 \right \rfloor }
\newcommand{\ceiling}[1]{\left \lceil #1 \right \rceil }
\newcommand{\interval}{I}
% \newcommand{\p}[2]{p_{#1}(#2)}
\newcommand{\ssketch}{\mathcmd{\mathsf{S}}}
\newcommand{\tsketch}{\mathcmd{\msgsettingsym\mathsf{S}}}
\newcommand{\trivsketch}{\mathcmd{\tsketch_{\emptystr}}}
\newcommand{\WREC}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}REC}}}
\newcommand{\AREC}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}REC}}}
\newcommand{\WUTIL}{\mathcmd{\pcnotionstyle{W\pcmathhyphen{}UTIL}}}
\newcommand{\AUTIL}{\mathcmd{\pcnotionstyle{A\pcmathhyphen{}UTIL}}}
\newcommand{\indexset}{I}
\newcommand{\topset}{Z_1^*}
\newcommand{\cachedist}{T}
\newcommand{\pwdis}{R}
\newcommand{\onbudget}{q}
\newcommand{\blacklist}{\textsf{B}}
\newcommand{\blacklistlen}{\alpha}
\newcommand{\plaintextstate}{\bar{\state}}
\newcommand{\typocutoff}{\delta}
\newcommand{\plfuprob}{\ensuremath{\nu}}

\def\ballweight{\ensuremath{e_{\tilde{\tau}}}}
\newcommand{\Adv}{\textnormal{\textsf{Adv}}}
\newcommand{\AdvOFFLINE}[1]{\Adv^{\footnotesize\textnormal{\textrm{offdist}}}_{\footnotesize #1}}
\newcommand{\AdvOFFLINEP}[1]{\Adv^{\overline{\footnotesize\textnormal{\textrm{{offdist}}}}}_{\footnotesize #1}}
\newcommand{\AdvOFFGUESS}[1]{\Adv^{\footnotesize\textnormal{\textrm{offguess}}}_{\footnotesize #1}}
\newcommand{\AdvONGUESS}[1]{\Adv^{{\footnotesize\textnormal{\textrm{onguess}}}}_{\footnotesize #1}}
\newcommand{\AdvONATTACK}[1]{\Adv^{\footnotesize\textnormal{\textrm{onattack}}}_{\footnotesize #1}}
\newcommand{\AdvRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{mk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvSRKROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{sk-ror}}}_{\footnotesize #1}}
\newcommand{\AdvROR}[1]{\Adv^{\footnotesize\textnormal{\textrm{ror}}}_{\footnotesize #1}}
\newcommand{\AdvROBUST}[1]{\Adv^{\footnotesize\textnormal{\textrm{rob}}}_{\footnotesize #1}}

\newcommand{\advantage}[3]{\pcnotionstyle{\Adv}^{#1}_{#2}(#3)}
\newcommand{\neighbourhood}[2]{N_{#1}({#2})}
\newcommand{\rhhdist}{Y}
\newcommand{\fullerhash}{z}
\newcommand{\errorball}[2]{{B}^{\errordist}_{#1}(#2)}
\newcommand{\f}{f}
\newcommand{\pwmaxlen}{\ell}
\newcommand{\indexi}{i}
\newcommand{\indexq}{q}
\newcommand{\indexx}{x}
\newcommand{\replace}{\textsf{replace}}
\newcommand{\vecca}{\vecc{a}}
\newcommand{\veccb}{\vecc{b}}
\newcommand{\veccv}{\vecc{v}}
\newcommand{\coins}{r}
\renewcommand{\state}{\ensuremath{\mathsf{s}}}
\newcommand{\win}{\mathsf{win}}
\newcommand{\Chk}{\textsf{Chk}}
\newcommand{\PChk}{\textsf{PChk}}
\newcommand{\indexh}{h}
\newcommand{\randomZ}{Z}
\newcommand{\Cache}{\textnormal{\textsf{Cache}}}
\newcommand{\WarmupCache}{\textnormal{\textsf{WarmupCache}}}
\newcommand{\CacheUpdate}{\textnormal{\textsf{CacheUpdt}}}
\newcommand{\CacheInit}{\textnormal{\textsf{CacheInit}}}
\newcommand{\cachestate}{\ensuremath{\mathtt{S}}\xspace}
\newcommand{\cachestatelen}{\ensuremath{\sigma}\xspace}
\newcommand{\CacheLRU}{\textnormal{\textsf{CacheLRU}}}
\newcommand{\CacheLRUUpdate}{\textnormal{\textsf{UpdateLRU}}}
\newcommand{\CacheLRUInit}{\textnormal{\textsf{InitLRU}}}


\newcommand{\zxcvbn}{\textnormal{\textsf{zxcvbn}}\xspace}
\newcommand{\bad}{\textnormal{\textsf{bad}}}
\newcommand{\wait}{z}
\newcommand{\PKE}{\textnormal{\textsf{PKE}}}
\newcommand{\pkegen}{\mathcal{K}}
\newcommand{\pkeenc}{\mathcal{E}}
\newcommand{\pkedec}{\mathcal{D}}
\newcommand{\pkectxtspace}{\mathcal{C}_{\pkeenc}}
\newcommand{\pk}{{pk}}
\newcommand{\sk}{{sk}}
\newcommand{\PBE}{\textnormal{\textsf{PBE}}}
\newcommand{\utility}{\textsf{Utility}}

\newcommand{\skegen}{\ensuremath{\mathsf{K}}}
\newcommand{\skeenc}{\ensuremath{\mathsf{E}}}
\newcommand{\skedec}{\ensuremath{\mathsf{D}}}
\newcommand{\skectxtspace}{\ensuremath{\mathcal{C}_{\skeenc}}}
\newcommand{\ske}{\textnormal{\textsf{SKE}}}
\newcommand{\SE}{\textnormal{\textsf{SE}}}
\newcommand{\sekg}{\mathcal{K}}
\newcommand{\seenc}{\mathcal{E}}
\newcommand{\sedec}{\mathcal{D}}
\newcommand{\saltlen}{{\ell_{\mathrm{salt}}}}

\newcommand{\skk}{\textnormal{\textsf{k}}}
\newcommand{\cipherske}{{c}}
\newcommand{\cipherpke}{{c}}
\newcommand{\SH}{\textnormal{\textsf{SH}}}
\newcommand{\FH}{\textnormal{\textsf{H}}}
\newcommand{\counter}{\textnormal{\textsf{Count}}}
\newcommand{\indexp}{p}
\newcommand{\ciphertextspace}{\mathcal{C}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\indexr}{r}
\newcommand{\vecc}[1]{\mathbf{#1}}
\newcommand{\sawait}{\overline{\sa}}
\newcommand{\skkwait}{\overline{\skk}}
\newcommand{\hwait}{\overline{\indexh}}
\newcommand{\randomY}{Y}
\newcommand{\indexm}{m}
\newcommand{\hashtable}[1]{H[#1]}
\newcommand{\SHlen}{k_1}
\newcommand{\FHlen}{k_2}
\newcommand{\valid}{\textnormal{\textsf{valid}}}
\newcommand{\skepsilon}{\epsilon_{ske}}
\newcommand{\pkepsilon}{\epsilon_{pke}}
\newcommand{\hybindex}{j}

\newcommand{\DL}{\textnormal{DL}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\indicator}{\mathbb{I}}
\newcommand{\cipherspace}{\mathcal{C}}
\newcommand{\pkemsgspace}{\mathcal{M}_\pkeenc}

\newcommand{\pkecipher}{c}
\newcommand{\skecipher}{{c}}
\newcommand{\pkemsg}{m}
\newcommand{\skemsg}{{m}}
\newcommand{\skemsgspace}{ \msgspace_{\skeenc}}
\newcommand{\upperb}{\alpha}

\newcommand{\ffbox}[1]{
   \setlength{\fboxsep}{-1\fboxrule}
   \fbox{\hspace{1.2pt}\strut#1\hspace{1.2pt}}}


\newcommand{\statespace}{S}
\newcommand{\targuess}{\textsf{TarGuess}}
\newcommand{\untarguess}{\textsf{UnTarGuess}}

\newcommand{\accept}{\texttt{accept}}
\newcommand{\reject}{\texttt{reject}}
\newcommand{\threshold}{\ensuremath{\tau}}
\newcommand{\clfthreshold}{\ensuremath{\theta}}
\newcommand{\far}{\ensuremath{\alpha}}
\newcommand{\frr}{\ensuremath{\beta}}
\newcommand{\fpr}{\ensuremath{\nu}}
\newcommand{\fnr}{\ensuremath{\gamma}}
\newcommand{\FPR}{\textrm{FPR}}
\newcommand{\FNR}{\textrm{FNR}}


\newcommand{\matchalgo}{\mathcal{L}}
\newcommand{\matchalgovec}{\mathcal{\mathbf{L}}_\sslen}
\def \score {\theta}
\newcommand{\indexjvec}{\ensuremath{\mathcmd{\mathbf{j}}\xspace}}
\def\k{k}
\newcommand{\add}{\funcfont{Add}}
\newcommand{\accuracy}{\funcfont{Accuracy}}
\def\acc{\delta}
\def \MS {\funcfont{MS}}
\def \MRec {\funcfont{MRec}}
\newcommand \MSt{\MS^{\matchalgo}_\sslen}
\newcommand \MRect{\MRec^{\matchalgo}_\sslen}
\def \nmatches {\ensuremath{l}}
\def \D{D}
\def \Dmod{\tilde{D}}
\def \mlen{n}
\def \sslen{t}
\def \secret{s}
\def \secretvec{\mathbf{s}}
\newcommand{\sketch}{{\funcfont{sketch}}}
\newcommand{\sketchval}{v}
\def \recover{\funcfont{recover}}
\def \verify{\funcfont{verify}}
\def \q{q}
\def\fp{\alpha}
\def\fn{\beta}
\def\tp{\gamma}
\newcommand{\one}{\ensuremath{\mathbbm{1}}}
\newcommand{\seclen}{\ell}
\newcommand{\Overify}{{\mathcal{O}_\funcfont{vrfy}}}
\newcommand{\Omatch}{\mathcal{O}_\funcfont{match}}
\newcommand{\ith}[2]{#1_{#2}}
\newcommand{\jth}[2]{#1^{#2}}
\newcommand{\mspacei}{\ith{\mspace}{i}}
\newcommand{\errori}{\ith{\error}{i}}
\newcommand{\matchalgoi}{\ith{\matchalgo}{i}}
\newcommand{\mvecbar}{\overline{\mvec}}
\newcommand{\mvectilde}{\tilde{\mvec}}
\newcommand{\angbrac}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\clf}{\mathcal{C}}
\newcommand{\clft}{\clf_\sslen}
\newcommand{\clfest}{\mathcal{\hat{\clf}}}
\newcommand{\clfq}[1]{{\clf^q_{#1}}}
\newcommand{\nclf}{r}
\newcommand{\oclf}{\omega}
\newcommand{\biosketch}{\funcfont{TenSketch}\xspace}
\newcommand{\tensketch}{\funcfont{TenSketch}\xspace}

\newcommand{\hvec}{\mathbf{h}}
\newcommand{\insertr}{\mathsf{insert{\scriptstyle\$}}}
\newcommand{\dbmsg}{\ensuremath{\mathcal{F}}}
\newcommand{\dbmsgs}{\ensuremath{\{\dbmsg_i\}}}
\newcommand{\dbid}{\mathcal{I}}
\newcommand{\db}{\ensuremath{D}}
% \newcommand{\dbs}{\ensuremath(\dbid,\{\dbmsg_i\})}
\newcommand{\dbs}{\ensuremath(\dbid,\dbmsg)}
\newcommand{\dbsprime}{\ensuremath(\dbid',\dbmsg')}
\newcommand{\dbsize}{N}
\def \dblen{N}
\def\mhat{\hat{\mvec}}
\def\findmatches{\funcfont{\footnotesize FindMatches$^{\matchalgo}$}}
\newcommand{\setss}[1]{\SS^\Delta_{#1}}
\newcommand{\setrec}[1]{\Rec^\Delta_{#1}}
\newcommand{\setsst}{\setss{\sslen}}
\newcommand{\setrect}{\setrec{\sslen}}
\newcommand{\costs}{{c_s}}
\newcommand{\costc}{{c_c}}
\NewDocumentCommand{\indseq}{ O{1} O{r} }{{#1}\ldots {#2}}
\newcommand{\seq}[2]{{{#1}_1,\ldots,{#1}_{#2}}}
\newcommand{\relu}{\funcfont{ReLu}}
\newcommand{\fcrelu}[1]{\funcfont{FC}_{\relu}^{#1}}
\newcommand{\gencliq}{\funcfont{GenTupIncr}}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

